Show Me Your Best Side: Characteristics of User-Preferred Perspectives for 3D Graph Drawings

The visual analysis of graphs in 3D has become increasingly popular, accelerated by the rise of immersive technology, such as augmented and virtual reality. Unlike 2D drawings, 3D graph layouts are highly viewpoint-dependent, making perspective selection critical for revealing structural and relational patterns. Despite its importance, there is limited empirical evidence guiding what constitutes an effective or preferred viewpoint from the user's perspective. In this paper, we present a systematic investigation into user-preferred viewpoints in 3D graph visualisations. We conducted a controlled study with 23 participants in a virtual reality environment, where users selected their most and least preferred viewpoints for 36 different graphs varying in size and layout. From this data, enriched by qualitative feedback, we distil common strategies underlying viewpoint choice. We further analyse the alignment of user preferences with classical 2D aesthetic criteria (e.g., Crossings), 3D-specific measures (e.g., Node-Node Occlusion), and introduce a novel measure capturing the perceivability of a graph's principal axes (Isometric Viewpoint Deviation). Our data-driven analysis indicates that Stress, Crossings, Gabriel Ratio, Edge-Node Overlap, and Isometric Viewpoint Deviation are key indicators of viewpoint preference. Beyond our findings, we contribute a publicly available dataset consisting of the graphs and computed aesthetic measures, supporting further research and the development of viewpoint evaluation measures for 3D graph drawing.

==> measure-table.tex <==

\begin{table}

\caption{[First results, not the final table]. The average values for 21 graph aesthetic measures for the 36 graphs (splitted into the judgements 'best' and 'worst) used in the evaluation. The values are normalised and higher values indicate higher quality. We calculated 21 measures, namely Node-Node Overlaps (\texttt{NNO}), the total area of Node-Node Overlaps (\texttt{NNOA}), Edge-Node Overlaps (\texttt{ENO}), the total area of Edge-Node Overlaps (\texttt{ENOA}), Node-Edge Overlaps (\texttt{NEO}), the total area of Node-Edge Overlaps (\texttt{NEOA}), the number of edge crossings (\texttt{CR}), stress (\texttt{ST}), crossing angular resolution (\texttt{CAR}), area (\texttt{AR}), aspect ratio (\texttt{ASP}), concentration (\texttt{CON}), node orthogonality (\texttt{NO}), Gabriel ratio (\texttt{GR}), angular resolution (\texttt{ANGR}), edge orthogonality (\texttt{EO}), edge length deviation (\texttt{ELD}), reflective edge symmetry (\texttt{ESR}), rotational edge symmetry (\texttt{ESO}), translational edge symmetry (\texttt{EST}), and the isometric projection measure (\texttt{ISO}).
}


\begin{tiny}
\def\arraystretch{1.2}
\setlength\tabcolsep{1pt}
\begin{tabular}{llccccccccccccccccccccccc}
\toprule
graph & answer & NNO & NNOA & ENO & ENOA & NEO & NEOA & CR & ST & CAR & AR & ASP & CON & NO & GR & ANGR & EO & ELD & ESR & ESO & EST & ISO \\
\midrule
can\_24 & Best & \cellcolor[HTML]{05713B} 0.98 & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{0E8244} 0.95 & \cellcolor[HTML]{09783F} 0.96 & \cellcolor[HTML]{08773E} 0.97 & \cellcolor[HTML]{0B7C41} 0.95 & \cellcolor[HTML]{08773E} 0.97 & \cellcolor[HTML]{18954E} 0.90 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{FB9F5A} 0.28 & \cellcolor[HTML]{66BD63} 0.80 & \cellcolor[HTML]{48AE5B} 0.84 & \cellcolor[HTML]{138B49} 0.92 & \cellcolor[HTML]{63BB62} 0.80 & \cellcolor[HTML]{FDBC6D} 0.33 & \cellcolor[HTML]{5DB860} 0.81 & \cellcolor[HTML]{FDC473} 0.35 & \cellcolor[HTML]{FDB063} 0.31 & \cellcolor[HTML]{FEE18D} 0.40 & \cellcolor[HTML]{C3E57C} 0.64 \\
can\_24 & Worst & \cellcolor[HTML]{FBFDB9} 0.51 & \cellcolor[HTML]{B3DE72} 0.68 & \cellcolor[HTML]{FDDC87} 0.39 & \cellcolor[HTML]{E1F297} 0.57 & \cellcolor[HTML]{FEE695} 0.42 & \cellcolor[HTML]{F6FBB3} 0.52 & \cellcolor[HTML]{E04430} 0.14 & \cellcolor[HTML]{D42D26} 0.10 & \cellcolor[HTML]{E75236} 0.16 & \cellcolor[HTML]{E95739} 0.17 & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{FEEA9D} 0.44 & \cellcolor[HTML]{E24932} 0.14 & \cellcolor[HTML]{F99354} 0.26 & \cellcolor[HTML]{FEE797} 0.42 & \cellcolor[HTML]{FEEA9D} 0.43 & \cellcolor[HTML]{FDD07D} 0.37 & \cellcolor[HTML]{FEFBB9} 0.49 & \cellcolor[HTML]{FEF9B5} 0.48 & \cellcolor[HTML]{F88E52} 0.25 \\
can\_96 & Best & \cellcolor[HTML]{279E53} 0.88 & \cellcolor[HTML]{0C7E42} 0.95 & \cellcolor[HTML]{54B45E} 0.82 & \cellcolor[HTML]{54B45E} 0.82 & \cellcolor[HTML]{6DC063} 0.79 & \cellcolor[HTML]{75C364} 0.78 & \cellcolor[HTML]{F9FCB7} 0.51 & \cellcolor[HTML]{B1DD71} 0.68 & \cellcolor[HTML]{DAEF8D} 0.59 & \cellcolor[HTML]{FDCA78} 0.36 & \cellcolor[HTML]{89CC66} 0.75 & \cellcolor[HTML]{B3DE72} 0.67 & \cellcolor[HTML]{DEF193} 0.58 & \cellcolor[HTML]{70C164} 0.78 & \cellcolor[HTML]{FEEDA1} 0.44 & \cellcolor[HTML]{FEEA9D} 0.44 & \cellcolor[HTML]{F9FCB7} 0.51 & \cellcolor[HTML]{FDC070} 0.34 & \cellcolor[HTML]{FDD884} 0.38 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{DDF091} 0.59 \\
can\_96 & Worst & \cellcolor[HTML]{BBE277} 0.66 & \cellcolor[HTML]{66BD63} 0.80 & \cellcolor[HTML]{9AD468} 0.72 & \cellcolor[HTML]{95D168} 0.72 & \cellcolor[HTML]{A9DA6B} 0.69 & \cellcolor[HTML]{9DD569} 0.71 & \cellcolor[HTML]{FDC675} 0.35 & \cellcolor[HTML]{FEE797} 0.42 & \cellcolor[HTML]{BBE277} 0.66 & \cellcolor[HTML]{FA9D59} 0.28 & \cellcolor[HTML]{E0F295} 0.58 & \cellcolor[HTML]{C3E57C} 0.64 & \cellcolor[HTML]{FEF2A9} 0.46 & \cellcolor[HTML]{BDE278} 0.66 & \cellcolor[HTML]{D9EF8B} 0.60 & \cellcolor[HTML]{FEEEA3} 0.45 & \cellcolor[HTML]{BDE278} 0.66 & \cellcolor[HTML]{FDC675} 0.35 & \cellcolor[HTML]{FEF8B3} 0.48 & \cellcolor[HTML]{FEF5AF} 0.47 & \cellcolor[HTML]{FEEC9F} 0.44 \\
dwt\_198 & Best & \cellcolor[HTML]{4EB15D} 0.83 & \cellcolor[HTML]{81C966} 0.76 & \cellcolor[HTML]{66BD63} 0.80 & \cellcolor[HTML]{7CC665} 0.77 & \cellcolor[HTML]{5DB860} 0.81 & \cellcolor[HTML]{6DC063} 0.79 & \cellcolor[HTML]{249D52} 0.89 & \cellcolor[HTML]{1E9A51} 0.89 & \cellcolor[HTML]{F88E52} 0.25 & \cellcolor[HTML]{FDC070} 0.34 & \cellcolor[HTML]{FDB466} 0.31 & \cellcolor[HTML]{E3F399} 0.57 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{66BD63} 0.80 & \cellcolor[HTML]{EAF6A3} 0.55 & \cellcolor[HTML]{F99354} 0.26 & \cellcolor[HTML]{CDE983} 0.62 & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{FDDC87} 0.39 & \cellcolor[HTML]{BFE37A} 0.65 & \cellcolor[HTML]{FEFAB7} 0.49 \\
dwt\_198 & Worst & \cellcolor[HTML]{A9DA6B} 0.69 & \cellcolor[HTML]{B9E176} 0.66 & \cellcolor[HTML]{F8FCB5} 0.52 & \cellcolor[HTML]{F3FAAF} 0.53 & \cellcolor[HTML]{F9FCB7} 0.52 & \cellcolor[HTML]{E6F49D} 0.56 & \cellcolor[HTML]{FEF5AF} 0.47 & \cellcolor[HTML]{72C264} 0.78 & \cellcolor[HTML]{FDD481} 0.38 & \cellcolor[HTML]{FDBA6B} 0.32 & \cellcolor[HTML]{FDC070} 0.34 & \cellcolor[HTML]{FEFDBB} 0.49 & \cellcolor[HTML]{FEF7B1} 0.48 & \cellcolor[HTML]{FDD481} 0.38 & \cellcolor[HTML]{7CC665} 0.76 & \cellcolor[HTML]{FB9F5A} 0.28 & \cellcolor[HTML]{F6FBB3} 0.52 & \cellcolor[HTML]{ECF7A5} 0.55 & \cellcolor[HTML]{DEF193} 0.58 & \cellcolor[HTML]{C1E47B} 0.65 & \cellcolor[HTML]{FDCA78} 0.36 \\
dwt\_209 & Best & \cellcolor[HTML]{18954E} 0.91 & \cellcolor[HTML]{219B51} 0.89 & \cellcolor[HTML]{36A557} 0.86 & \cellcolor[HTML]{219B51} 0.89 & \cellcolor[HTML]{1B9850} 0.90 & \cellcolor[HTML]{36A557} 0.86 & \cellcolor[HTML]{42AB5A} 0.84 & \cellcolor[HTML]{148D4A} 0.92 & \cellcolor[HTML]{FDD07D} 0.37 & \cellcolor[HTML]{CBE881} 0.63 & \cellcolor[HTML]{F88E52} 0.25 & \cellcolor[HTML]{C1E47B} 0.65 & \cellcolor[HTML]{279E53} 0.88 & \cellcolor[HTML]{3CA858} 0.85 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{F9FCB7} 0.51 & \cellcolor[HTML]{D3EC87} 0.61 & \cellcolor[HTML]{D5ED88} 0.61 & \cellcolor[HTML]{DBF08F} 0.59 & \cellcolor[HTML]{DEF193} 0.58 & \cellcolor[HTML]{EDF7A7} 0.54 \\
dwt\_209 & Worst & \cellcolor[HTML]{FEF2A9} 0.46 & \cellcolor[HTML]{ECF7A5} 0.55 & \cellcolor[HTML]{FDC675} 0.35 & \cellcolor[HTML]{E0F295} 0.58 & \cellcolor[HTML]{FEE391} 0.41 & \cellcolor[HTML]{E9F5A1} 0.56 & \cellcolor[HTML]{EE613D} 0.18 & \cellcolor[HTML]{E75236} 0.16 & \cellcolor[HTML]{F6814C} 0.23 & \cellcolor[HTML]{F47245} 0.21 & \cellcolor[HTML]{7FC765} 0.76 & \cellcolor[HTML]{BBE277} 0.66 & \cellcolor[HTML]{FEFDBB} 0.49 & \cellcolor[HTML]{F16840} 0.19 & \cellcolor[HTML]{FDC272} 0.34 & \cellcolor[HTML]{F5FAB1} 0.53 & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{8ECE67} 0.74 & \cellcolor[HTML]{3CA858} 0.85 & \cellcolor[HTML]{30A255} 0.87 & \cellcolor[HTML]{F0653F} 0.19 \\
grafo10183.100 & Best & \cellcolor[HTML]{4EB15D} 0.83 & \cellcolor[HTML]{60BA61} 0.81 & \cellcolor[HTML]{2DA154} 0.87 & \cellcolor[HTML]{60BA61} 0.81 & \cellcolor[HTML]{48AE5B} 0.84 & \cellcolor[HTML]{60BA61} 0.81 & \cellcolor[HTML]{5DB860} 0.81 & \cellcolor[HTML]{72C264} 0.78 & \cellcolor[HTML]{FDD884} 0.38 & \cellcolor[HTML]{F6FBB3} 0.52 & \cellcolor[HTML]{FEFBB9} 0.49 & \cellcolor[HTML]{95D168} 0.72 & \cellcolor[HTML]{7CC665} 0.76 & \cellcolor[HTML]{C3E57C} 0.64 & \cellcolor[HTML]{7CC665} 0.76 & \cellcolor[HTML]{FDCA78} 0.36 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{FDB668} 0.32 & \cellcolor[HTML]{FEE695} 0.42 & \cellcolor[HTML]{FDC877} 0.35 & \cellcolor[HTML]{FEF9B5} 0.48 \\
grafo10183.100 & Worst & \cellcolor[HTML]{DAEF8D} 0.59 & \cellcolor[HTML]{CDE983} 0.62 & \cellcolor[HTML]{C5E67E} 0.64 & \cellcolor[HTML]{E4F49B} 0.57 & \cellcolor[HTML]{B9E176} 0.66 & \cellcolor[HTML]{ADDC6E} 0.68 & \cellcolor[HTML]{FEEC9F} 0.44 & \cellcolor[HTML]{F7864E} 0.24 & \cellcolor[HTML]{FBA25B} 0.28 & \cellcolor[HTML]{FEE18D} 0.40 & \cellcolor[HTML]{F3FAAF} 0.53 & \cellcolor[HTML]{A7D96A} 0.70 & \cellcolor[HTML]{BFE37A} 0.65 & \cellcolor[HTML]{F67E4B} 0.23 & \cellcolor[HTML]{FEE28F} 0.41 & \cellcolor[HTML]{FDDA86} 0.39 & \cellcolor[HTML]{FDC877} 0.35 & \cellcolor[HTML]{F99555} 0.26 & \cellcolor[HTML]{DBF08F} 0.59 & \cellcolor[HTML]{FDBA6B} 0.32 & \cellcolor[HTML]{FDCC7A} 0.36 \\
grafo2347.20 & Best & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{016937} 0.99 & \cellcolor[HTML]{036D39} 0.99 & \cellcolor[HTML]{0C7E42} 0.95 & \cellcolor[HTML]{1E9A51} 0.89 & \cellcolor[HTML]{FDB466} 0.32 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{FDD682} 0.38 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{81C966} 0.76 & \cellcolor[HTML]{118847} 0.93 & \cellcolor[HTML]{2DA154} 0.87 & \cellcolor[HTML]{FDB668} 0.32 & \cellcolor[HTML]{2DA154} 0.87 & \cellcolor[HTML]{FDBE6E} 0.33 & \cellcolor[HTML]{E44B33} 0.15 & \cellcolor[HTML]{F89053} 0.26 & \cellcolor[HTML]{75C364} 0.77 \\
grafo2347.20 & Worst & \cellcolor[HTML]{FDB466} 0.31 & \cellcolor[HTML]{EAF6A3} 0.55 & \cellcolor[HTML]{F0653F} 0.19 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{FDCE7C} 0.37 & \cellcolor[HTML]{FDDE89} 0.40 & \cellcolor[HTML]{F88B51} 0.25 & \cellcolor[HTML]{E14631} 0.14 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{FB9F5A} 0.28 & \cellcolor[HTML]{FEF3AB} 0.46 & \cellcolor[HTML]{FEE99B} 0.43 & \cellcolor[HTML]{F0F9AB} 0.54 & \cellcolor[HTML]{EE613D} 0.18 & \cellcolor[HTML]{FDC070} 0.34 & \cellcolor[HTML]{FEE695} 0.42 & \cellcolor[HTML]{ED5E3C} 0.18 & \cellcolor[HTML]{75C364} 0.77 & \cellcolor[HTML]{A9DA6B} 0.69 & \cellcolor[HTML]{FEFBB9} 0.49 & \cellcolor[HTML]{E14631} 0.14 \\
grafo5640.50 & Best & \cellcolor[HTML]{4BAF5C} 0.83 & \cellcolor[HTML]{30A255} 0.87 & \cellcolor[HTML]{4BAF5C} 0.84 & \cellcolor[HTML]{51B25D} 0.83 & \cellcolor[HTML]{A7D96A} 0.70 & \cellcolor[HTML]{C9E880} 0.63 & \cellcolor[HTML]{3FAA59} 0.85 & \cellcolor[HTML]{45AD5A} 0.84 & \cellcolor[HTML]{F7834D} 0.24 & \cellcolor[HTML]{FDD884} 0.39 & \cellcolor[HTML]{FEE18D} 0.40 & \cellcolor[HTML]{93D067} 0.73 & \cellcolor[HTML]{BDE278} 0.65 & \cellcolor[HTML]{E1F297} 0.57 & \cellcolor[HTML]{C1E47B} 0.65 & \cellcolor[HTML]{FDCE7C} 0.37 & \cellcolor[HTML]{BDE278} 0.66 & \cellcolor[HTML]{FDB668} 0.32 & \cellcolor[HTML]{FEE18D} 0.41 & \cellcolor[HTML]{FDC272} 0.34 & \cellcolor[HTML]{BBE277} 0.66 \\
grafo5640.50 & Worst & \cellcolor[HTML]{A2D769} 0.70 & \cellcolor[HTML]{7AC565} 0.77 & \cellcolor[HTML]{E9F5A1} 0.56 & \cellcolor[HTML]{E0F295} 0.58 & \cellcolor[HTML]{F5FAB1} 0.53 & \cellcolor[HTML]{F2F9AD} 0.53 & \cellcolor[HTML]{FEEDA1} 0.44 & \cellcolor[HTML]{FBA55C} 0.29 & \cellcolor[HTML]{F88B51} 0.25 & \cellcolor[HTML]{FDD07D} 0.37 & \cellcolor[HTML]{FEF9B5} 0.48 & \cellcolor[HTML]{A2D769} 0.70 & \cellcolor[HTML]{D7EE89} 0.61 & \cellcolor[HTML]{F67E4B} 0.23 & \cellcolor[HTML]{4EB15D} 0.83 & \cellcolor[HTML]{FDDA86} 0.39 & \cellcolor[HTML]{A7D96A} 0.70 & \cellcolor[HTML]{FEEA9D} 0.43 & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{FEF5AF} 0.47 & \cellcolor[HTML]{FEF5AF} 0.47 \\
layered\_2\_20\_36 & Best & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{08773E} 0.97 & \cellcolor[HTML]{06733C} 0.97 & \cellcolor[HTML]{0A7A40} 0.96 & \cellcolor[HTML]{09783F} 0.96 & \cellcolor[HTML]{3CA858} 0.85 & \cellcolor[HTML]{72C264} 0.78 & \cellcolor[HTML]{FDC473} 0.35 & \cellcolor[HTML]{FEE797} 0.42 & \cellcolor[HTML]{E0F295} 0.58 & \cellcolor[HTML]{7FC765} 0.76 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{EFF8A9} 0.54 & \cellcolor[HTML]{77C464} 0.77 & \cellcolor[HTML]{FEF7B1} 0.47 & \cellcolor[HTML]{DAEF8D} 0.60 & \cellcolor[HTML]{FDB86A} 0.32 & \cellcolor[HTML]{E04430} 0.13 & \cellcolor[HTML]{F47245} 0.21 & \cellcolor[HTML]{D1EB85} 0.61 \\
layered\_2\_20\_36 & Worst & \cellcolor[HTML]{93D067} 0.73 & \cellcolor[HTML]{72C264} 0.78 & \cellcolor[HTML]{BFE37A} 0.65 & \cellcolor[HTML]{8ECE67} 0.74 & \cellcolor[HTML]{BFE37A} 0.65 & \cellcolor[HTML]{9AD468} 0.72 & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{FDD481} 0.38 & \cellcolor[HTML]{FDB466} 0.32 & \cellcolor[HTML]{F26A41} 0.20 & \cellcolor[HTML]{D5ED88} 0.61 & \cellcolor[HTML]{FCFEBB} 0.51 & \cellcolor[HTML]{FEF7B1} 0.48 & \cellcolor[HTML]{F16840} 0.19 & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{FEFBB9} 0.49 & \cellcolor[HTML]{FEF9B5} 0.48 & \cellcolor[HTML]{FDD481} 0.38 & \cellcolor[HTML]{FA9D59} 0.27 & \cellcolor[HTML]{FDB86A} 0.32 & \cellcolor[HTML]{F57446} 0.21 \\
layered\_2\_20\_38 & Best & \cellcolor[HTML]{06733C} 0.98 & \cellcolor[HTML]{016937} 0.99 & \cellcolor[HTML]{0F8445} 0.94 & \cellcolor[HTML]{08773E} 0.97 & \cellcolor[HTML]{148D4A} 0.92 & \cellcolor[HTML]{158F4B} 0.92 & \cellcolor[HTML]{3CA858} 0.85 & \cellcolor[HTML]{51B25D} 0.82 & \cellcolor[HTML]{FDDA86} 0.39 & \cellcolor[HTML]{F6FBB3} 0.52 & \cellcolor[HTML]{E4F49B} 0.57 & \cellcolor[HTML]{7FC765} 0.76 & \cellcolor[HTML]{60BA61} 0.81 & \cellcolor[HTML]{FEFAB7} 0.49 & \cellcolor[HTML]{84CA66} 0.75 & \cellcolor[HTML]{FEEC9F} 0.44 & \cellcolor[HTML]{F5FAB1} 0.52 & \cellcolor[HTML]{FDD07D} 0.37 & \cellcolor[HTML]{F99555} 0.26 & \cellcolor[HTML]{FBA55C} 0.29 & \cellcolor[HTML]{BBE277} 0.66 \\
layered\_2\_20\_38 & Worst & \cellcolor[HTML]{9DD569} 0.71 & \cellcolor[HTML]{84CA66} 0.75 & \cellcolor[HTML]{C3E57C} 0.64 & \cellcolor[HTML]{95D168} 0.73 & \cellcolor[HTML]{D1EB85} 0.62 & \cellcolor[HTML]{C9E880} 0.63 & \cellcolor[HTML]{CDE983} 0.62 & \cellcolor[HTML]{D3EC87} 0.61 & \cellcolor[HTML]{FDC675} 0.35 & \cellcolor[HTML]{FB9F5A} 0.28 & \cellcolor[HTML]{FEEFA5} 0.45 & \cellcolor[HTML]{DEF193} 0.58 & \cellcolor[HTML]{F2F9AD} 0.53 & \cellcolor[HTML]{FDB063} 0.31 & \cellcolor[HTML]{F9FCB7} 0.51 & \cellcolor[HTML]{FEEC9F} 0.44 & \cellcolor[HTML]{C7E77F} 0.63 & \cellcolor[HTML]{FEE493} 0.42 & \cellcolor[HTML]{FDBC6D} 0.33 & \cellcolor[HTML]{FEF9B5} 0.48 & \cellcolor[HTML]{FDC272} 0.34 \\
layered\_2\_20\_40 & Best & \cellcolor[HTML]{026B38} 0.99 & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{128948} 0.93 & \cellcolor[HTML]{0C7E42} 0.95 & \cellcolor[HTML]{18954E} 0.90 & \cellcolor[HTML]{138B49} 0.93 & \cellcolor[HTML]{BFE37A} 0.65 & \cellcolor[HTML]{CBE881} 0.63 & \cellcolor[HTML]{FEFDBB} 0.49 & \cellcolor[HTML]{FEE695} 0.42 & \cellcolor[HTML]{C1E47B} 0.65 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{B1DD71} 0.68 & \cellcolor[HTML]{F3FAAF} 0.53 & \cellcolor[HTML]{75C364} 0.78 & \cellcolor[HTML]{FDC675} 0.35 & \cellcolor[HTML]{FEEA9D} 0.43 & \cellcolor[HTML]{FDDC87} 0.39 & \cellcolor[HTML]{F99555} 0.26 & \cellcolor[HTML]{F57446} 0.21 & \cellcolor[HTML]{FEFBB9} 0.49 \\
layered\_2\_20\_40 & Worst & \cellcolor[HTML]{6BBF63} 0.79 & \cellcolor[HTML]{42AB5A} 0.84 & \cellcolor[HTML]{C1E47B} 0.65 & \cellcolor[HTML]{C7E77F} 0.64 & \cellcolor[HTML]{E9F5A1} 0.56 & \cellcolor[HTML]{CDE983} 0.62 & \cellcolor[HTML]{E0F295} 0.58 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{FEFAB7} 0.48 & \cellcolor[HTML]{FDCE7C} 0.36 & \cellcolor[HTML]{E4F49B} 0.57 & \cellcolor[HTML]{BBE277} 0.66 & \cellcolor[HTML]{CDE983} 0.62 & \cellcolor[HTML]{FEE899} 0.43 & \cellcolor[HTML]{EFF8A9} 0.54 & \cellcolor[HTML]{FDDC87} 0.39 & \cellcolor[HTML]{F8FCB5} 0.52 & \cellcolor[HTML]{FEEDA1} 0.44 & \cellcolor[HTML]{FA9856} 0.27 & \cellcolor[HTML]{FDD27F} 0.37 & \cellcolor[HTML]{FEEA9D} 0.44 \\
layered\_2\_50\_101 & Best & \cellcolor[HTML]{0E8244} 0.94 & \cellcolor[HTML]{06733C} 0.97 & \cellcolor[HTML]{1B9850} 0.90 & \cellcolor[HTML]{148D4A} 0.92 & \cellcolor[HTML]{19974F} 0.90 & \cellcolor[HTML]{1E9A51} 0.89 & \cellcolor[HTML]{98D268} 0.72 & \cellcolor[HTML]{F3FAAF} 0.53 & \cellcolor[HTML]{DEF193} 0.59 & \cellcolor[HTML]{FEE99B} 0.43 & \cellcolor[HTML]{F6FBB3} 0.52 & \cellcolor[HTML]{9AD468} 0.72 & \cellcolor[HTML]{B5DF73} 0.67 & \cellcolor[HTML]{E6F49D} 0.56 & \cellcolor[HTML]{54B45E} 0.82 & \cellcolor[HTML]{FDD481} 0.38 & \cellcolor[HTML]{FDCC7A} 0.36 & \cellcolor[HTML]{FEE99B} 0.43 & \cellcolor[HTML]{FDD884} 0.39 & \cellcolor[HTML]{FDB668} 0.32 & \cellcolor[HTML]{EFF8A9} 0.54 \\
layered\_2\_50\_101 & Worst & \cellcolor[HTML]{6DC063} 0.79 & \cellcolor[HTML]{4BAF5C} 0.83 & \cellcolor[HTML]{75C364} 0.78 & \cellcolor[HTML]{6BBF63} 0.79 & \cellcolor[HTML]{A2D769} 0.71 & \cellcolor[HTML]{90CF67} 0.73 & \cellcolor[HTML]{9DD569} 0.71 & \cellcolor[HTML]{A2D769} 0.71 & \cellcolor[HTML]{FEEDA1} 0.44 & \cellcolor[HTML]{FDC070} 0.34 & \cellcolor[HTML]{FDDC87} 0.39 & \cellcolor[HTML]{AFDC6F} 0.68 & \cellcolor[HTML]{E1F297} 0.58 & \cellcolor[HTML]{B1DD71} 0.68 & \cellcolor[HTML]{8BCD67} 0.74 & \cellcolor[HTML]{FEF3AB} 0.46 & \cellcolor[HTML]{9AD468} 0.72 & \cellcolor[HTML]{FDBE6E} 0.33 & \cellcolor[HTML]{FDD481} 0.38 & \cellcolor[HTML]{FDD682} 0.38 & \cellcolor[HTML]{F67C4A} 0.23 \\
layered\_2\_50\_102 & Best & \cellcolor[HTML]{0A7A40} 0.96 & \cellcolor[HTML]{046F3A} 0.98 & \cellcolor[HTML]{1B9850} 0.90 & \cellcolor[HTML]{0F8445} 0.94 & \cellcolor[HTML]{17934D} 0.91 & \cellcolor[HTML]{16914C} 0.91 & \cellcolor[HTML]{ABDB6D} 0.69 & \cellcolor[HTML]{FEEC9F} 0.44 & \cellcolor[HTML]{F9FCB7} 0.51 & \cellcolor[HTML]{FDDE89} 0.40 & \cellcolor[HTML]{B7E075} 0.67 & \cellcolor[HTML]{63BB62} 0.80 & \cellcolor[HTML]{9AD468} 0.72 & \cellcolor[HTML]{DEF193} 0.59 & \cellcolor[HTML]{8BCD67} 0.74 & \cellcolor[HTML]{F26A41} 0.20 & \cellcolor[HTML]{FDDA86} 0.39 & \cellcolor[HTML]{FEF9B5} 0.48 & \cellcolor[HTML]{F9FCB7} 0.51 & \cellcolor[HTML]{FDB86A} 0.32 & \cellcolor[HTML]{FEFDBB} 0.50 \\
layered\_2\_50\_102 & Worst & \cellcolor[HTML]{8ECE67} 0.74 & \cellcolor[HTML]{7CC665} 0.76 & \cellcolor[HTML]{BDE278} 0.66 & \cellcolor[HTML]{9FD669} 0.71 & \cellcolor[HTML]{D9EF8B} 0.60 & \cellcolor[HTML]{CBE881} 0.63 & \cellcolor[HTML]{B3DE72} 0.67 & \cellcolor[HTML]{EFF8A9} 0.54 & \cellcolor[HTML]{FEEC9F} 0.44 & \cellcolor[HTML]{FDCA78} 0.36 & \cellcolor[HTML]{BDE278} 0.66 & \cellcolor[HTML]{9FD669} 0.71 & \cellcolor[HTML]{B7E075} 0.67 & \cellcolor[HTML]{F3FAAF} 0.53 & \cellcolor[HTML]{DEF193} 0.58 & \cellcolor[HTML]{F7864E} 0.24 & \cellcolor[HTML]{EAF6A3} 0.55 & \cellcolor[HTML]{FEF3AB} 0.46 & \cellcolor[HTML]{F6FBB3} 0.52 & \cellcolor[HTML]{FEF2A9} 0.46 & \cellcolor[HTML]{FEF7B1} 0.47 \\
layered\_2\_50\_93 & Best & \cellcolor[HTML]{06733C} 0.98 & \cellcolor[HTML]{016937} 0.99 & \cellcolor[HTML]{118847} 0.93 & \cellcolor[HTML]{118847} 0.93 & \cellcolor[HTML]{0F8445} 0.94 & \cellcolor[HTML]{158F4B} 0.92 & \cellcolor[HTML]{C1E47B} 0.65 & \cellcolor[HTML]{EFF8A9} 0.54 & \cellcolor[HTML]{A4D869} 0.70 & \cellcolor[HTML]{FDD481} 0.38 & \cellcolor[HTML]{EDF7A7} 0.54 & \cellcolor[HTML]{57B55F} 0.82 & \cellcolor[HTML]{CDE983} 0.62 & \cellcolor[HTML]{D9EF8B} 0.60 & \cellcolor[HTML]{5DB860} 0.81 & \cellcolor[HTML]{FEF9B5} 0.48 & \cellcolor[HTML]{FDD682} 0.38 & \cellcolor[HTML]{E0F295} 0.58 & \cellcolor[HTML]{FDAE61} 0.30 & \cellcolor[HTML]{F7894F} 0.24 & \cellcolor[HTML]{FBA25B} 0.28 \\
layered\_2\_50\_93 & Worst & \cellcolor[HTML]{9FD669} 0.71 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{A9DA6B} 0.69 & \cellcolor[HTML]{9DD569} 0.71 & \cellcolor[HTML]{A4D869} 0.70 & \cellcolor[HTML]{9DD569} 0.71 & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{CDE983} 0.62 & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{FCAC60} 0.30 & \cellcolor[HTML]{FDC473} 0.34 & \cellcolor[HTML]{B7E075} 0.67 & \cellcolor[HTML]{E9F5A1} 0.56 & \cellcolor[HTML]{F0F9AB} 0.54 & \cellcolor[HTML]{B1DD71} 0.68 & \cellcolor[HTML]{FEF8B3} 0.48 & \cellcolor[HTML]{C7E77F} 0.64 & \cellcolor[HTML]{C5E67E} 0.64 & \cellcolor[HTML]{FDB466} 0.31 & \cellcolor[HTML]{FDD884} 0.38 & \cellcolor[HTML]{FDC877} 0.35 \\
layered\_3\_100\_207 & Best & \cellcolor[HTML]{42AB5A} 0.85 & \cellcolor[HTML]{1E9A51} 0.89 & \cellcolor[HTML]{39A757} 0.86 & \cellcolor[HTML]{3FAA59} 0.85 & \cellcolor[HTML]{42AB5A} 0.85 & \cellcolor[HTML]{7AC565} 0.77 & \cellcolor[HTML]{7FC765} 0.76 & \cellcolor[HTML]{7AC565} 0.77 & \cellcolor[HTML]{D83328} 0.11 & \cellcolor[HTML]{FEE08B} 0.40 & \cellcolor[HTML]{ECF7A5} 0.55 & \cellcolor[HTML]{98D268} 0.72 & \cellcolor[HTML]{D9EF8B} 0.60 & \cellcolor[HTML]{F9FCB7} 0.51 & \cellcolor[HTML]{72C264} 0.78 & \cellcolor[HTML]{FA9A58} 0.27 & \cellcolor[HTML]{F99354} 0.26 & \cellcolor[HTML]{BBE277} 0.66 & \cellcolor[HTML]{D5ED88} 0.61 & \cellcolor[HTML]{F0653F} 0.19 & \cellcolor[HTML]{FEFAB7} 0.49 \\
layered\_3\_100\_207 & Worst & \cellcolor[HTML]{77C464} 0.77 & \cellcolor[HTML]{6BBF63} 0.79 & \cellcolor[HTML]{ABDB6D} 0.69 & \cellcolor[HTML]{ADDC6E} 0.68 & \cellcolor[HTML]{A9DA6B} 0.69 & \cellcolor[HTML]{C7E77F} 0.63 & \cellcolor[HTML]{F46D43} 0.20 & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{CC2526} 0.08 & \cellcolor[HTML]{F7894F} 0.25 & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{4BAF5C} 0.83 & \cellcolor[HTML]{FEE695} 0.42 & \cellcolor[HTML]{EF633E} 0.19 & \cellcolor[HTML]{219B51} 0.89 & \cellcolor[HTML]{F67C4A} 0.22 & \cellcolor[HTML]{3CA858} 0.85 & \cellcolor[HTML]{C7E77F} 0.64 & \cellcolor[HTML]{9DD569} 0.71 & \cellcolor[HTML]{F99555} 0.26 & \cellcolor[HTML]{EE613D} 0.18 \\
layered\_3\_100\_253 & Best & \cellcolor[HTML]{39A757} 0.86 & \cellcolor[HTML]{148D4A} 0.92 & \cellcolor[HTML]{279E53} 0.88 & \cellcolor[HTML]{2A9F54} 0.88 & \cellcolor[HTML]{36A557} 0.86 & \cellcolor[HTML]{39A757} 0.86 & \cellcolor[HTML]{CBE881} 0.63 & \cellcolor[HTML]{BDE278} 0.66 & \cellcolor[HTML]{A4D869} 0.70 & \cellcolor[HTML]{FEEC9F} 0.44 & \cellcolor[HTML]{93D067} 0.73 & \cellcolor[HTML]{84CA66} 0.75 & \cellcolor[HTML]{B3DE72} 0.67 & \cellcolor[HTML]{C1E47B} 0.65 & \cellcolor[HTML]{66BD63} 0.80 & \cellcolor[HTML]{EA593A} 0.17 & \cellcolor[HTML]{FDB466} 0.31 & \cellcolor[HTML]{E14631} 0.14 & \cellcolor[HTML]{FDD481} 0.38 & \cellcolor[HTML]{E65035} 0.15 & \cellcolor[HTML]{E7F59F} 0.56 \\
layered\_3\_100\_253 & Worst & \cellcolor[HTML]{60BA61} 0.80 & \cellcolor[HTML]{30A255} 0.87 & \cellcolor[HTML]{AFDC6F} 0.68 & \cellcolor[HTML]{93D067} 0.73 & \cellcolor[HTML]{B7E075} 0.66 & \cellcolor[HTML]{A2D769} 0.70 & \cellcolor[HTML]{FA9D59} 0.28 & \cellcolor[HTML]{F57948} 0.22 & \cellcolor[HTML]{E1F297} 0.58 & \cellcolor[HTML]{FDB86A} 0.32 & \cellcolor[HTML]{FEF9B5} 0.48 & \cellcolor[HTML]{48AE5B} 0.84 & \cellcolor[HTML]{F0F9AB} 0.54 & \cellcolor[HTML]{EA593A} 0.17 & \cellcolor[HTML]{1E9A51} 0.89 & \cellcolor[HTML]{EA593A} 0.17 & \cellcolor[HTML]{6DC063} 0.79 & \cellcolor[HTML]{E75236} 0.16 & \cellcolor[HTML]{FEFDBB} 0.49 & \cellcolor[HTML]{F7894F} 0.24 & \cellcolor[HTML]{F6814C} 0.23 \\
layered\_3\_100\_284 & Best & \cellcolor[HTML]{36A557} 0.86 & \cellcolor[HTML]{158F4B} 0.92 & \cellcolor[HTML]{128948} 0.93 & \cellcolor[HTML]{33A456} 0.86 & \cellcolor[HTML]{39A757} 0.86 & \cellcolor[HTML]{45AD5A} 0.84 & \cellcolor[HTML]{39A757} 0.86 & \cellcolor[HTML]{1B9850} 0.90 & \cellcolor[HTML]{FDBA6B} 0.32 & \cellcolor[HTML]{DAEF8D} 0.60 & \cellcolor[HTML]{B3DE72} 0.67 & \cellcolor[HTML]{B9E176} 0.66 & \cellcolor[HTML]{6BBF63} 0.79 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{AFDC6F} 0.68 & \cellcolor[HTML]{FEFAB7} 0.49 & \cellcolor[HTML]{EF633E} 0.18 & \cellcolor[HTML]{8ECE67} 0.73 & \cellcolor[HTML]{FDDA86} 0.39 & \cellcolor[HTML]{FDD884} 0.38 & \cellcolor[HTML]{E1F297} 0.58 \\
layered\_3\_100\_284 & Worst & \cellcolor[HTML]{8BCD67} 0.74 & \cellcolor[HTML]{63BB62} 0.80 & \cellcolor[HTML]{ABDB6D} 0.69 & \cellcolor[HTML]{B9E176} 0.66 & \cellcolor[HTML]{B9E176} 0.66 & \cellcolor[HTML]{9FD669} 0.71 & \cellcolor[HTML]{FCA75E} 0.29 & \cellcolor[HTML]{FDBC6D} 0.33 & \cellcolor[HTML]{FEEA9D} 0.44 & \cellcolor[HTML]{FEF9B5} 0.48 & \cellcolor[HTML]{FEF8B3} 0.48 & \cellcolor[HTML]{A7D96A} 0.70 & \cellcolor[HTML]{ABDB6D} 0.69 & \cellcolor[HTML]{E65035} 0.15 & \cellcolor[HTML]{ADDC6E} 0.68 & \cellcolor[HTML]{FEF8B3} 0.48 & \cellcolor[HTML]{7FC765} 0.76 & \cellcolor[HTML]{8BCD67} 0.74 & \cellcolor[HTML]{EFF8A9} 0.54 & \cellcolor[HTML]{F0F9AB} 0.54 & \cellcolor[HTML]{F26A41} 0.20 \\
layered\_3\_200\_431 & Best & \cellcolor[HTML]{1B9850} 0.90 & \cellcolor[HTML]{158F4B} 0.92 & \cellcolor[HTML]{30A255} 0.87 & \cellcolor[HTML]{45AD5A} 0.84 & \cellcolor[HTML]{249D52} 0.89 & \cellcolor[HTML]{54B45E} 0.82 & \cellcolor[HTML]{5AB760} 0.81 & \cellcolor[HTML]{72C264} 0.78 & \cellcolor[HTML]{FDBC6D} 0.33 & \cellcolor[HTML]{FEFAB7} 0.48 & \cellcolor[HTML]{F0F9AB} 0.54 & \cellcolor[HTML]{8ECE67} 0.74 & \cellcolor[HTML]{AFDC6F} 0.68 & \cellcolor[HTML]{A7D96A} 0.70 & \cellcolor[HTML]{39A757} 0.86 & \cellcolor[HTML]{FA9D59} 0.27 & \cellcolor[HTML]{FCAA5F} 0.30 & \cellcolor[HTML]{C82126} 0.07 & \cellcolor[HTML]{F6814C} 0.23 & \cellcolor[HTML]{FA9D59} 0.28 & \cellcolor[HTML]{B1DD71} 0.68 \\
layered\_3\_200\_431 & Worst & \cellcolor[HTML]{2A9F54} 0.88 & \cellcolor[HTML]{2A9F54} 0.88 & \cellcolor[HTML]{B1DD71} 0.68 & \cellcolor[HTML]{D3EC87} 0.61 & \cellcolor[HTML]{6BBF63} 0.79 & \cellcolor[HTML]{9AD468} 0.72 & \cellcolor[HTML]{ED5E3C} 0.18 & \cellcolor[HTML]{FDC675} 0.35 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{FDCC7A} 0.36 & \cellcolor[HTML]{FDD07D} 0.37 & \cellcolor[HTML]{5AB760} 0.82 & \cellcolor[HTML]{E6F49D} 0.56 & \cellcolor[HTML]{E54D34} 0.15 & \cellcolor[HTML]{1E9A51} 0.89 & \cellcolor[HTML]{FDB063} 0.31 & \cellcolor[HTML]{2DA154} 0.87 & \cellcolor[HTML]{C82126} 0.07 & \cellcolor[HTML]{FDBE6E} 0.34 & \cellcolor[HTML]{FEE18D} 0.40 & \cellcolor[HTML]{DE3F2E} 0.13 \\
layered\_3\_200\_487 & Best & \cellcolor[HTML]{5DB860} 0.81 & \cellcolor[HTML]{33A456} 0.86 & \cellcolor[HTML]{5AB760} 0.82 & \cellcolor[HTML]{42AB5A} 0.84 & \cellcolor[HTML]{5AB760} 0.81 & \cellcolor[HTML]{66BD63} 0.80 & \cellcolor[HTML]{279E53} 0.88 & \cellcolor[HTML]{95D168} 0.73 & \cellcolor[HTML]{ECF7A5} 0.55 & \cellcolor[HTML]{FEFAB7} 0.49 & \cellcolor[HTML]{C7E77F} 0.64 & \cellcolor[HTML]{DAEF8D} 0.59 & \cellcolor[HTML]{93D067} 0.73 & \cellcolor[HTML]{8ECE67} 0.74 & \cellcolor[HTML]{9AD468} 0.72 & \cellcolor[HTML]{FDD07D} 0.37 & \cellcolor[HTML]{F57446} 0.21 & \cellcolor[HTML]{57B55F} 0.82 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{F7864E} 0.24 & \cellcolor[HTML]{ECF7A5} 0.55 \\
layered\_3\_200\_487 & Worst & \cellcolor[HTML]{48AE5B} 0.84 & \cellcolor[HTML]{42AB5A} 0.85 & \cellcolor[HTML]{DBF08F} 0.59 & \cellcolor[HTML]{C3E57C} 0.64 & \cellcolor[HTML]{C9E880} 0.63 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{FDB668} 0.32 & \cellcolor[HTML]{FEEA9D} 0.43 & \cellcolor[HTML]{72C264} 0.78 & \cellcolor[HTML]{FA9D59} 0.27 & \cellcolor[HTML]{FEEA9D} 0.44 & \cellcolor[HTML]{7CC665} 0.76 & \cellcolor[HTML]{F5FAB1} 0.53 & \cellcolor[HTML]{F7834D} 0.24 & \cellcolor[HTML]{3CA858} 0.85 & \cellcolor[HTML]{FDD07D} 0.37 & \cellcolor[HTML]{66BD63} 0.80 & \cellcolor[HTML]{219B51} 0.89 & \cellcolor[HTML]{57B55F} 0.82 & \cellcolor[HTML]{FDCE7C} 0.36 & \cellcolor[HTML]{F67E4B} 0.23 \\
layered\_3\_200\_508 & Best & \cellcolor[HTML]{7AC565} 0.77 & \cellcolor[HTML]{4BAF5C} 0.83 & \cellcolor[HTML]{2DA154} 0.87 & \cellcolor[HTML]{57B55F} 0.82 & \cellcolor[HTML]{60BA61} 0.81 & \cellcolor[HTML]{57B55F} 0.82 & \cellcolor[HTML]{36A557} 0.86 & \cellcolor[HTML]{42AB5A} 0.84 & \cellcolor[HTML]{FEF7B1} 0.48 & \cellcolor[HTML]{FEE695} 0.42 & \cellcolor[HTML]{F5FAB1} 0.52 & \cellcolor[HTML]{D9EF8B} 0.60 & \cellcolor[HTML]{ADDC6E} 0.69 & \cellcolor[HTML]{E6F49D} 0.57 & \cellcolor[HTML]{81C966} 0.76 & \cellcolor[HTML]{FEE493} 0.42 & \cellcolor[HTML]{F0653F} 0.19 & \cellcolor[HTML]{D73127} 0.10 & \cellcolor[HTML]{D9EF8B} 0.60 & \cellcolor[HTML]{FEFDBB} 0.49 & \cellcolor[HTML]{D5ED88} 0.61 \\
layered\_3\_200\_508 & Worst & \cellcolor[HTML]{3CA858} 0.85 & \cellcolor[HTML]{39A757} 0.86 & \cellcolor[HTML]{84CA66} 0.75 & \cellcolor[HTML]{A4D869} 0.70 & \cellcolor[HTML]{DAEF8D} 0.60 & \cellcolor[HTML]{C7E77F} 0.64 & \cellcolor[HTML]{FDB265} 0.31 & \cellcolor[HTML]{FDC272} 0.34 & \cellcolor[HTML]{E0F295} 0.58 & \cellcolor[HTML]{FCAC60} 0.30 & \cellcolor[HTML]{EAF6A3} 0.55 & \cellcolor[HTML]{6BBF63} 0.79 & \cellcolor[HTML]{DEF193} 0.58 & \cellcolor[HTML]{C62026} 0.07 & \cellcolor[HTML]{18954E} 0.90 & \cellcolor[HTML]{FEE899} 0.43 & \cellcolor[HTML]{219B51} 0.89 & \cellcolor[HTML]{D62F26} 0.10 & \cellcolor[HTML]{98D268} 0.72 & \cellcolor[HTML]{F9FCB7} 0.51 & \cellcolor[HTML]{F7894F} 0.24 \\
mesh1em1 & Best & \cellcolor[HTML]{1B9850} 0.90 & \cellcolor[HTML]{128948} 0.93 & \cellcolor[HTML]{219B51} 0.89 & \cellcolor[HTML]{30A255} 0.87 & \cellcolor[HTML]{279E53} 0.88 & \cellcolor[HTML]{33A456} 0.87 & \cellcolor[HTML]{54B45E} 0.82 & \cellcolor[HTML]{93D067} 0.73 & \cellcolor[HTML]{C1E47B} 0.64 & \cellcolor[HTML]{FEEDA1} 0.44 & \cellcolor[HTML]{F5FAB1} 0.52 & \cellcolor[HTML]{60BA61} 0.81 & \cellcolor[HTML]{D1EB85} 0.61 & \cellcolor[HTML]{7AC565} 0.77 & \cellcolor[HTML]{A4D869} 0.70 & \cellcolor[HTML]{FDD07D} 0.37 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{A9DA6B} 0.69 & \cellcolor[HTML]{E9F5A1} 0.56 & \cellcolor[HTML]{FEE797} 0.42 & \cellcolor[HTML]{FDB668} 0.32 \\
mesh1em1 & Worst & \cellcolor[HTML]{A4D869} 0.70 & \cellcolor[HTML]{77C464} 0.77 & \cellcolor[HTML]{B9E176} 0.66 & \cellcolor[HTML]{C1E47B} 0.64 & \cellcolor[HTML]{E6F49D} 0.57 & \cellcolor[HTML]{C7E77F} 0.64 & \cellcolor[HTML]{ECF7A5} 0.55 & \cellcolor[HTML]{FEEDA1} 0.44 & \cellcolor[HTML]{FDD27F} 0.37 & \cellcolor[HTML]{FB9F5A} 0.28 & \cellcolor[HTML]{D7EE89} 0.60 & \cellcolor[HTML]{DDF091} 0.59 & \cellcolor[HTML]{FEEDA1} 0.44 & \cellcolor[HTML]{FEE28F} 0.41 & \cellcolor[HTML]{FEE899} 0.43 & \cellcolor[HTML]{FDD27F} 0.37 & \cellcolor[HTML]{FEE391} 0.41 & \cellcolor[HTML]{9DD569} 0.71 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{FEEEA3} 0.45 & \cellcolor[HTML]{FEFBB9} 0.49 \\
sem\_0\_20\_16 & Best & \cellcolor[HTML]{138B49} 0.92 & \cellcolor[HTML]{0D8043} 0.95 & \cellcolor[HTML]{09783F} 0.96 & \cellcolor[HTML]{09783F} 0.96 & \cellcolor[HTML]{249D52} 0.88 & \cellcolor[HTML]{36A557} 0.86 & \cellcolor[HTML]{89CC66} 0.74 & \cellcolor[HTML]{7AC565} 0.77 & \cellcolor[HTML]{89CC66} 0.74 & \cellcolor[HTML]{F9FCB7} 0.51 & \cellcolor[HTML]{E6F49D} 0.56 & \cellcolor[HTML]{70C164} 0.78 & \cellcolor[HTML]{5DB860} 0.81 & \cellcolor[HTML]{C5E67E} 0.64 & \cellcolor[HTML]{B7E075} 0.67 & \cellcolor[HTML]{FDB668} 0.32 & \cellcolor[HTML]{7FC765} 0.76 & \cellcolor[HTML]{FDB668} 0.32 & \cellcolor[HTML]{FCA75E} 0.29 & \cellcolor[HTML]{D22B26} 0.09 & \cellcolor[HTML]{FEF1A7} 0.46 \\
sem\_0\_20\_16 & Worst & \cellcolor[HTML]{B3DE72} 0.67 & \cellcolor[HTML]{9FD669} 0.71 & \cellcolor[HTML]{9DD569} 0.71 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{D1EB85} 0.62 & \cellcolor[HTML]{FEFBB9} 0.49 & \cellcolor[HTML]{77C464} 0.77 & \cellcolor[HTML]{FDDC87} 0.39 & \cellcolor[HTML]{FEF2A9} 0.46 & \cellcolor[HTML]{F99555} 0.26 & \cellcolor[HTML]{FDD07D} 0.37 & \cellcolor[HTML]{FEFBB9} 0.49 & \cellcolor[HTML]{F5FAB1} 0.52 & \cellcolor[HTML]{FB9F5A} 0.28 & \cellcolor[HTML]{B1DD71} 0.68 & \cellcolor[HTML]{FDD07D} 0.37 & \cellcolor[HTML]{F0F9AB} 0.54 & \cellcolor[HTML]{EF633E} 0.18 & \cellcolor[HTML]{FDB063} 0.31 & \cellcolor[HTML]{F46D43} 0.20 & \cellcolor[HTML]{FDC272} 0.34 \\
sem\_0\_50\_100 & Best & \cellcolor[HTML]{148D4A} 0.92 & \cellcolor[HTML]{219B51} 0.89 & \cellcolor[HTML]{108646} 0.93 & \cellcolor[HTML]{19974F} 0.90 & \cellcolor[HTML]{17934D} 0.91 & \cellcolor[HTML]{17934D} 0.91 & \cellcolor[HTML]{51B25D} 0.83 & \cellcolor[HTML]{57B55F} 0.82 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{B5DF73} 0.67 & \cellcolor[HTML]{54B45E} 0.82 & \cellcolor[HTML]{158F4B} 0.92 & \cellcolor[HTML]{A9DA6B} 0.69 & \cellcolor[HTML]{75C364} 0.78 & \cellcolor[HTML]{FEF9B5} 0.48 & \cellcolor[HTML]{90CF67} 0.73 & \cellcolor[HTML]{B1DD71} 0.68 & \cellcolor[HTML]{FB9F5A} 0.28 & \cellcolor[HTML]{FDB466} 0.32 & \cellcolor[HTML]{BFE37A} 0.65 \\
sem\_0\_50\_100 & Worst & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{F5FAB1} 0.52 & \cellcolor[HTML]{FBFDB9} 0.51 & \cellcolor[HTML]{F6FBB3} 0.52 & \cellcolor[HTML]{CDE983} 0.62 & \cellcolor[HTML]{B5DF73} 0.67 & \cellcolor[HTML]{FEE99B} 0.43 & \cellcolor[HTML]{FEE18D} 0.40 & \cellcolor[HTML]{F7894F} 0.24 & \cellcolor[HTML]{F6814C} 0.23 & \cellcolor[HTML]{FEE391} 0.41 & \cellcolor[HTML]{E4F49B} 0.57 & \cellcolor[HTML]{D9EF8B} 0.60 & \cellcolor[HTML]{FDDA86} 0.39 & \cellcolor[HTML]{DBF08F} 0.59 & \cellcolor[HTML]{EAF6A3} 0.55 & \cellcolor[HTML]{FDDC87} 0.39 & \cellcolor[HTML]{9DD569} 0.71 & \cellcolor[HTML]{FDCA78} 0.36 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{FDB466} 0.32 \\
sem\_1\_20\_22 & Best & \cellcolor[HTML]{09783F} 0.96 & \cellcolor[HTML]{036D39} 0.98 & \cellcolor[HTML]{0E8244} 0.94 & \cellcolor[HTML]{0C7E42} 0.95 & \cellcolor[HTML]{45AD5A} 0.84 & \cellcolor[HTML]{2A9F54} 0.88 & \cellcolor[HTML]{68BE63} 0.80 & \cellcolor[HTML]{81C966} 0.75 & \cellcolor[HTML]{FEE899} 0.43 & \cellcolor[HTML]{B1DD71} 0.68 & \cellcolor[HTML]{E1F297} 0.58 & \cellcolor[HTML]{84CA66} 0.75 & \cellcolor[HTML]{16914C} 0.91 & \cellcolor[HTML]{FDD27F} 0.37 & \cellcolor[HTML]{68BE63} 0.80 & \cellcolor[HTML]{FDDA86} 0.39 & \cellcolor[HTML]{57B55F} 0.82 & \cellcolor[HTML]{FCAC60} 0.30 & \cellcolor[HTML]{FEEFA5} 0.45 & \cellcolor[HTML]{FDD481} 0.38 & \cellcolor[HTML]{C5E67E} 0.64 \\
sem\_1\_20\_22 & Worst & \cellcolor[HTML]{DDF091} 0.59 & \cellcolor[HTML]{ABDB6D} 0.69 & \cellcolor[HTML]{E1F297} 0.57 & \cellcolor[HTML]{C9E880} 0.63 & \cellcolor[HTML]{FDD884} 0.38 & \cellcolor[HTML]{E1F297} 0.58 & \cellcolor[HTML]{E1F297} 0.58 & \cellcolor[HTML]{FEFDBB} 0.49 & \cellcolor[HTML]{FA9856} 0.27 & \cellcolor[HTML]{F7834D} 0.24 & \cellcolor[HTML]{FDCA78} 0.36 & \cellcolor[HTML]{D5ED88} 0.61 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{E95739} 0.16 & \cellcolor[HTML]{FEE18D} 0.41 & \cellcolor[HTML]{FDD07D} 0.37 & \cellcolor[HTML]{9FD669} 0.71 & \cellcolor[HTML]{FDD682} 0.38 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{B5DF73} 0.67 & \cellcolor[HTML]{FDD682} 0.38 \\
sem\_1\_50\_100 & Best & \cellcolor[HTML]{19974F} 0.90 & \cellcolor[HTML]{118847} 0.93 & \cellcolor[HTML]{108646} 0.94 & \cellcolor[HTML]{138B49} 0.93 & \cellcolor[HTML]{33A456} 0.87 & \cellcolor[HTML]{57B55F} 0.82 & \cellcolor[HTML]{138B49} 0.92 & \cellcolor[HTML]{6DC063} 0.79 & \cellcolor[HTML]{90CF67} 0.73 & \cellcolor[HTML]{DBF08F} 0.59 & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{C3E57C} 0.64 & \cellcolor[HTML]{2DA154} 0.87 & \cellcolor[HTML]{75C364} 0.77 & \cellcolor[HTML]{60BA61} 0.81 & \cellcolor[HTML]{FEF3AB} 0.46 & \cellcolor[HTML]{42AB5A} 0.85 & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{F89053} 0.26 & \cellcolor[HTML]{EE613D} 0.18 & \cellcolor[HTML]{A9DA6B} 0.69 \\
sem\_1\_50\_100 & Worst & \cellcolor[HTML]{FEE99B} 0.43 & \cellcolor[HTML]{FDBC6D} 0.33 & \cellcolor[HTML]{FEE695} 0.42 & \cellcolor[HTML]{FCFEBB} 0.50 & \cellcolor[HTML]{FEE18D} 0.40 & \cellcolor[HTML]{FEEC9F} 0.44 & \cellcolor[HTML]{FDC473} 0.34 & \cellcolor[HTML]{FBA55C} 0.29 & \cellcolor[HTML]{FDCA78} 0.36 & \cellcolor[HTML]{E44B33} 0.14 & \cellcolor[HTML]{FCAC60} 0.30 & \cellcolor[HTML]{FEE493} 0.41 & \cellcolor[HTML]{FEE899} 0.43 & \cellcolor[HTML]{F0653F} 0.19 & \cellcolor[HTML]{B5DF73} 0.67 & \cellcolor[HTML]{F3FAAF} 0.53 & \cellcolor[HTML]{E4F49B} 0.57 & \cellcolor[HTML]{FEFAB7} 0.49 & \cellcolor[HTML]{FDB86A} 0.32 & \cellcolor[HTML]{FDD481} 0.38 & \cellcolor[HTML]{FDBE6E} 0.33 \\
sem\_2\_100\_144 & Best & \cellcolor[HTML]{77C464} 0.77 & \cellcolor[HTML]{5DB860} 0.81 & \cellcolor[HTML]{4EB15D} 0.83 & \cellcolor[HTML]{48AE5B} 0.84 & \cellcolor[HTML]{45AD5A} 0.84 & \cellcolor[HTML]{98D268} 0.72 & \cellcolor[HTML]{68BE63} 0.79 & \cellcolor[HTML]{81C966} 0.76 & \cellcolor[HTML]{E6F49D} 0.57 & \cellcolor[HTML]{FEEFA5} 0.45 & \cellcolor[HTML]{EDF7A7} 0.55 & \cellcolor[HTML]{D5ED88} 0.61 & \cellcolor[HTML]{C3E57C} 0.64 & \cellcolor[HTML]{F5FAB1} 0.53 & \cellcolor[HTML]{7FC765} 0.76 & \cellcolor[HTML]{FEE797} 0.42 & \cellcolor[HTML]{CBE881} 0.63 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{FDAE61} 0.30 & \cellcolor[HTML]{FEEFA5} 0.45 & \cellcolor[HTML]{E7F59F} 0.56 \\
sem\_2\_100\_144 & Worst & \cellcolor[HTML]{A7D96A} 0.70 & \cellcolor[HTML]{93D067} 0.73 & \cellcolor[HTML]{E6F49D} 0.57 & \cellcolor[HTML]{C3E57C} 0.64 & \cellcolor[HTML]{54B45E} 0.82 & \cellcolor[HTML]{ABDB6D} 0.69 & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{F8FCB5} 0.52 & \cellcolor[HTML]{FDB063} 0.31 & \cellcolor[HTML]{FDB86A} 0.32 & \cellcolor[HTML]{B7E075} 0.67 & \cellcolor[HTML]{FEF5AF} 0.47 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{FDC272} 0.34 & \cellcolor[HTML]{C1E47B} 0.65 & \cellcolor[HTML]{FEEC9F} 0.44 & \cellcolor[HTML]{C9E880} 0.63 & \cellcolor[HTML]{ADDC6E} 0.69 & \cellcolor[HTML]{FEE28F} 0.41 & \cellcolor[HTML]{C5E67E} 0.64 & \cellcolor[HTML]{FDDA86} 0.39 \\
sem\_2\_20\_19 & Best & \cellcolor[HTML]{09783F} 0.96 & \cellcolor[HTML]{046F3A} 0.98 & \cellcolor[HTML]{108646} 0.93 & \cellcolor[HTML]{158F4B} 0.92 & \cellcolor[HTML]{54B45E} 0.82 & \cellcolor[HTML]{5DB860} 0.81 & \cellcolor[HTML]{7CC665} 0.76 & \cellcolor[HTML]{18954E} 0.90 & \cellcolor[HTML]{FEE391} 0.41 & \cellcolor[HTML]{FEFBB9} 0.49 & \cellcolor[HTML]{DAEF8D} 0.60 & \cellcolor[HTML]{7CC665} 0.76 & \cellcolor[HTML]{36A557} 0.86 & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{89CC66} 0.74 & \cellcolor[HTML]{FEE493} 0.42 & \cellcolor[HTML]{4EB15D} 0.83 & \cellcolor[HTML]{FDBA6B} 0.32 & \cellcolor[HTML]{FDCE7C} 0.36 & \cellcolor[HTML]{E85538} 0.16 & \cellcolor[HTML]{FDCE7C} 0.36 \\
sem\_2\_20\_19 & Worst & \cellcolor[HTML]{BBE277} 0.66 & \cellcolor[HTML]{98D268} 0.72 & \cellcolor[HTML]{E9F5A1} 0.56 & \cellcolor[HTML]{EAF6A3} 0.55 & \cellcolor[HTML]{D9EF8B} 0.60 & \cellcolor[HTML]{E4F49B} 0.57 & \cellcolor[HTML]{95D168} 0.72 & \cellcolor[HTML]{FEF8B3} 0.48 & \cellcolor[HTML]{FEE08B} 0.40 & \cellcolor[HTML]{E95739} 0.17 & \cellcolor[HTML]{F7834D} 0.24 & \cellcolor[HTML]{D5ED88} 0.61 & \cellcolor[HTML]{F3FAAF} 0.53 & \cellcolor[HTML]{F7834D} 0.23 & \cellcolor[HTML]{D5ED88} 0.61 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{FDB466} 0.31 & \cellcolor[HTML]{FDCA78} 0.36 & \cellcolor[HTML]{FDCE7C} 0.37 & \cellcolor[HTML]{FDB063} 0.31 \\
sem\_2\_50\_100 & Best & \cellcolor[HTML]{36A557} 0.86 & \cellcolor[HTML]{2A9F54} 0.88 & \cellcolor[HTML]{33A456} 0.87 & \cellcolor[HTML]{219B51} 0.89 & \cellcolor[HTML]{68BE63} 0.80 & \cellcolor[HTML]{39A757} 0.86 & \cellcolor[HTML]{D3EC87} 0.61 & \cellcolor[HTML]{66BD63} 0.80 & \cellcolor[HTML]{B1DD71} 0.68 & \cellcolor[HTML]{DEF193} 0.59 & \cellcolor[HTML]{C5E67E} 0.64 & \cellcolor[HTML]{66BD63} 0.80 & \cellcolor[HTML]{1E9A51} 0.89 & \cellcolor[HTML]{C9E880} 0.63 & \cellcolor[HTML]{3CA858} 0.85 & \cellcolor[HTML]{FEE18D} 0.41 & \cellcolor[HTML]{158F4B} 0.92 & \cellcolor[HTML]{B7E075} 0.67 & \cellcolor[HTML]{EAF6A3} 0.55 & \cellcolor[HTML]{FBA25B} 0.28 & \cellcolor[HTML]{A7D96A} 0.70 \\
sem\_2\_50\_100 & Worst & \cellcolor[HTML]{BBE277} 0.66 & \cellcolor[HTML]{B1DD71} 0.68 & \cellcolor[HTML]{FDC473} 0.35 & \cellcolor[HTML]{FEFBB9} 0.49 & \cellcolor[HTML]{F6FBB3} 0.52 & \cellcolor[HTML]{B3DE72} 0.67 & \cellcolor[HTML]{B7E075} 0.67 & \cellcolor[HTML]{FDC272} 0.34 & \cellcolor[HTML]{FCAA5F} 0.29 & \cellcolor[HTML]{F88B51} 0.25 & \cellcolor[HTML]{FDD481} 0.38 & \cellcolor[HTML]{C9E880} 0.63 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{FBA25B} 0.28 & \cellcolor[HTML]{DBF08F} 0.59 & \cellcolor[HTML]{FEF5AF} 0.47 & \cellcolor[HTML]{FEF2A9} 0.46 & \cellcolor[HTML]{FDC473} 0.34 & \cellcolor[HTML]{B3DE72} 0.67 & \cellcolor[HTML]{FEE797} 0.42 & \cellcolor[HTML]{FEE08B} 0.40 \\
sem\_3\_100\_137 & Best & \cellcolor[HTML]{7AC565} 0.77 & \cellcolor[HTML]{45AD5A} 0.84 & \cellcolor[HTML]{33A456} 0.87 & \cellcolor[HTML]{1E9A51} 0.89 & \cellcolor[HTML]{4BAF5C} 0.83 & \cellcolor[HTML]{81C966} 0.75 & \cellcolor[HTML]{77C464} 0.77 & \cellcolor[HTML]{6DC063} 0.79 & \cellcolor[HTML]{FEEEA3} 0.45 & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{7AC565} 0.77 & \cellcolor[HTML]{A7D96A} 0.70 & \cellcolor[HTML]{95D168} 0.72 & \cellcolor[HTML]{FEF8B3} 0.48 & \cellcolor[HTML]{DAEF8D} 0.60 & \cellcolor[HTML]{63BB62} 0.80 & \cellcolor[HTML]{F99354} 0.26 & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{FEEFA5} 0.45 & \cellcolor[HTML]{C7E77F} 0.63 \\
sem\_3\_100\_137 & Worst & \cellcolor[HTML]{D9EF8B} 0.60 & \cellcolor[HTML]{90CF67} 0.73 & \cellcolor[HTML]{FEF5AF} 0.47 & \cellcolor[HTML]{D7EE89} 0.60 & \cellcolor[HTML]{5DB860} 0.81 & \cellcolor[HTML]{9FD669} 0.71 & \cellcolor[HTML]{FEEFA5} 0.45 & \cellcolor[HTML]{FDB063} 0.31 & \cellcolor[HTML]{FDBC6D} 0.33 & \cellcolor[HTML]{FA9D59} 0.27 & \cellcolor[HTML]{C9E880} 0.63 & \cellcolor[HTML]{C1E47B} 0.65 & \cellcolor[HTML]{FEFBB9} 0.49 & \cellcolor[HTML]{FDB466} 0.31 & \cellcolor[HTML]{B5DF73} 0.67 & \cellcolor[HTML]{F5FAB1} 0.53 & \cellcolor[HTML]{63BB62} 0.80 & \cellcolor[HTML]{FEEC9F} 0.44 & \cellcolor[HTML]{EAF6A3} 0.55 & \cellcolor[HTML]{FCFEBB} 0.51 & \cellcolor[HTML]{F99354} 0.26 \\
sem\_5\_200\_194 & Best & \cellcolor[HTML]{0C7E42} 0.95 & \cellcolor[HTML]{148D4A} 0.92 & \cellcolor[HTML]{18954E} 0.91 & \cellcolor[HTML]{33A456} 0.87 & \cellcolor[HTML]{90CF67} 0.73 & \cellcolor[HTML]{77C464} 0.77 & \cellcolor[HTML]{9DD569} 0.71 & \cellcolor[HTML]{0C7E42} 0.95 & \cellcolor[HTML]{F5FAB1} 0.52 & \cellcolor[HTML]{E9F5A1} 0.56 & \cellcolor[HTML]{FDCC7A} 0.36 & \cellcolor[HTML]{DAEF8D} 0.60 & \cellcolor[HTML]{6DC063} 0.79 & \cellcolor[HTML]{8ECE67} 0.74 & \cellcolor[HTML]{ADDC6E} 0.68 & \cellcolor[HTML]{FDD884} 0.38 & \cellcolor[HTML]{7FC765} 0.76 & \cellcolor[HTML]{5AB760} 0.82 & \cellcolor[HTML]{70C164} 0.78 & \cellcolor[HTML]{FDD682} 0.38 & \cellcolor[HTML]{FBFDB9} 0.51 \\
sem\_5\_200\_194 & Worst & \cellcolor[HTML]{E3F399} 0.57 & \cellcolor[HTML]{E0F295} 0.58 & \cellcolor[HTML]{FEFAB7} 0.48 & \cellcolor[HTML]{E9F5A1} 0.56 & \cellcolor[HTML]{DEF193} 0.58 & \cellcolor[HTML]{A7D96A} 0.70 & \cellcolor[HTML]{FEFBB9} 0.49 & \cellcolor[HTML]{FEF7B1} 0.47 & \cellcolor[HTML]{FDBE6E} 0.33 & \cellcolor[HTML]{F6814C} 0.23 & \cellcolor[HTML]{FDC473} 0.35 & \cellcolor[HTML]{C9E880} 0.63 & \cellcolor[HTML]{FEEFA5} 0.45 & \cellcolor[HTML]{FDB063} 0.31 & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{FEE797} 0.43 & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{30A255} 0.87 & \cellcolor[HTML]{30A255} 0.87 & \cellcolor[HTML]{BBE277} 0.66 & \cellcolor[HTML]{FBA25B} 0.28 \\
sem\_6\_200\_202 & Best & \cellcolor[HTML]{0A7A40} 0.96 & \cellcolor[HTML]{128948} 0.93 & \cellcolor[HTML]{57B55F} 0.82 & \cellcolor[HTML]{3CA858} 0.85 & \cellcolor[HTML]{5AB760} 0.81 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{F3FAAF} 0.53 & \cellcolor[HTML]{7CC665} 0.77 & \cellcolor[HTML]{F57747} 0.22 & \cellcolor[HTML]{F3FAAF} 0.53 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{66BD63} 0.80 & \cellcolor[HTML]{75C364} 0.78 & \cellcolor[HTML]{FEE493} 0.42 & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{FBFDB9} 0.51 & \cellcolor[HTML]{FEE18D} 0.40 & \cellcolor[HTML]{7FC765} 0.76 & \cellcolor[HTML]{F16840} 0.19 & \cellcolor[HTML]{FEF8B3} 0.48 & \cellcolor[HTML]{FEF9B5} 0.48 \\
sem\_6\_200\_202 & Worst & \cellcolor[HTML]{F9FCB7} 0.51 & \cellcolor[HTML]{E0F295} 0.58 & \cellcolor[HTML]{E7F59F} 0.56 & \cellcolor[HTML]{B9E176} 0.66 & \cellcolor[HTML]{ADDC6E} 0.69 & \cellcolor[HTML]{9AD468} 0.71 & \cellcolor[HTML]{E6F49D} 0.56 & \cellcolor[HTML]{5AB760} 0.81 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{FDB063} 0.31 & \cellcolor[HTML]{FEE18D} 0.41 & \cellcolor[HTML]{AFDC6F} 0.68 & \cellcolor[HTML]{F8FCB5} 0.52 & \cellcolor[HTML]{FEE99B} 0.43 & \cellcolor[HTML]{95D168} 0.73 & \cellcolor[HTML]{FCFEBB} 0.51 & \cellcolor[HTML]{A7D96A} 0.70 & \cellcolor[HTML]{17934D} 0.91 & \cellcolor[HTML]{FDC473} 0.35 & \cellcolor[HTML]{C5E67E} 0.64 & \cellcolor[HTML]{FA9A58} 0.27 \\
sem\_9\_100\_131 & Best & \cellcolor[HTML]{4BAF5C} 0.83 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{219B51} 0.89 & \cellcolor[HTML]{1E9A51} 0.89 & \cellcolor[HTML]{CBE881} 0.63 & \cellcolor[HTML]{DBF08F} 0.59 & \cellcolor[HTML]{57B55F} 0.82 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{F9FCB7} 0.51 & \cellcolor[HTML]{E1F297} 0.58 & \cellcolor[HTML]{FDD682} 0.38 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{90CF67} 0.73 & \cellcolor[HTML]{84CA66} 0.75 & \cellcolor[HTML]{B1DD71} 0.68 & \cellcolor[HTML]{FDD481} 0.38 & \cellcolor[HTML]{9FD669} 0.71 & \cellcolor[HTML]{B1DD71} 0.68 & \cellcolor[HTML]{FEE18D} 0.40 & \cellcolor[HTML]{FCAC60} 0.30 & \cellcolor[HTML]{E1F297} 0.58 \\
sem\_9\_100\_131 & Worst & \cellcolor[HTML]{A9DA6B} 0.69 & \cellcolor[HTML]{E9F5A1} 0.56 & \cellcolor[HTML]{FEE28F} 0.41 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{219B51} 0.89 & \cellcolor[HTML]{7FC765} 0.76 & \cellcolor[HTML]{8BCD67} 0.74 & \cellcolor[HTML]{FDC675} 0.35 & \cellcolor[HTML]{FDB265} 0.31 & \cellcolor[HTML]{FDB86A} 0.32 & \cellcolor[HTML]{D9EF8B} 0.60 & \cellcolor[HTML]{DAEF8D} 0.59 & \cellcolor[HTML]{FEFDBB} 0.49 & \cellcolor[HTML]{F0653F} 0.19 & \cellcolor[HTML]{AFDC6F} 0.68 & \cellcolor[HTML]{FDC473} 0.35 & \cellcolor[HTML]{C1E47B} 0.65 & \cellcolor[HTML]{B7E075} 0.67 & \cellcolor[HTML]{FEF3AB} 0.46 & \cellcolor[HTML]{FB9F5A} 0.28 & \cellcolor[HTML]{FDB265} 0.31 \\
sem\_9\_200\_150 & Best & \cellcolor[HTML]{108646} 0.94 & \cellcolor[HTML]{128948} 0.93 & \cellcolor[HTML]{54B45E} 0.82 & \cellcolor[HTML]{4BAF5C} 0.83 & \cellcolor[HTML]{5DB860} 0.81 & \cellcolor[HTML]{5DB860} 0.81 & \cellcolor[HTML]{249D52} 0.89 & \cellcolor[HTML]{158F4B} 0.91 & \cellcolor[HTML]{FDC877} 0.35 & \cellcolor[HTML]{F6FBB3} 0.52 & \cellcolor[HTML]{FDC272} 0.34 & \cellcolor[HTML]{93D067} 0.73 & \cellcolor[HTML]{6DC063} 0.79 & \cellcolor[HTML]{77C464} 0.77 & \cellcolor[HTML]{93D067} 0.73 & \cellcolor[HTML]{FDD27F} 0.37 & \cellcolor[HTML]{17934D} 0.91 & \cellcolor[HTML]{EF633E} 0.18 & \cellcolor[HTML]{FA9A58} 0.27 & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{E0F295} 0.58 \\
sem\_9\_200\_150 & Worst & \cellcolor[HTML]{FDCA78} 0.36 & \cellcolor[HTML]{F3FAAF} 0.53 & \cellcolor[HTML]{FEFDBB} 0.50 & \cellcolor[HTML]{C9E880} 0.63 & \cellcolor[HTML]{F9FCB7} 0.52 & \cellcolor[HTML]{9DD569} 0.71 & \cellcolor[HTML]{F7834D} 0.24 & \cellcolor[HTML]{F88E52} 0.25 & \cellcolor[HTML]{A2D769} 0.71 & \cellcolor[HTML]{F16840} 0.19 & \cellcolor[HTML]{FEE391} 0.41 & \cellcolor[HTML]{D9EF8B} 0.60 & \cellcolor[HTML]{FEE899} 0.43 & \cellcolor[HTML]{F46F44} 0.20 & \cellcolor[HTML]{BBE277} 0.66 & \cellcolor[HTML]{FDD682} 0.38 & \cellcolor[HTML]{FDC473} 0.35 & \cellcolor[HTML]{FDC070} 0.34 & \cellcolor[HTML]{E0F295} 0.58 & \cellcolor[HTML]{30A255} 0.87 & \cellcolor[HTML]{F57747} 0.22 \\
tree\_100\_2 & Best & \cellcolor[HTML]{9AD468} 0.72 & \cellcolor[HTML]{A4D869} 0.70 & \cellcolor[HTML]{86CB66} 0.75 & \cellcolor[HTML]{70C164} 0.78 & \cellcolor[HTML]{68BE63} 0.79 & \cellcolor[HTML]{77C464} 0.77 & \cellcolor[HTML]{138B49} 0.93 & \cellcolor[HTML]{138B49} 0.92 & \cellcolor[HTML]{F0653F} 0.19 & \cellcolor[HTML]{ECF7A5} 0.55 & \cellcolor[HTML]{FEE99B} 0.43 & \cellcolor[HTML]{9DD569} 0.71 & \cellcolor[HTML]{6DC063} 0.79 & \cellcolor[HTML]{7AC565} 0.77 & \cellcolor[HTML]{FEE695} 0.42 & \cellcolor[HTML]{FEF2A9} 0.46 & \cellcolor[HTML]{FEEC9F} 0.44 & \cellcolor[HTML]{6DC063} 0.79 & \cellcolor[HTML]{FDDC87} 0.39 & \cellcolor[HTML]{FDBA6B} 0.33 & \cellcolor[HTML]{F0F9AB} 0.54 \\
tree\_100\_2 & Worst & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{FEF5AF} 0.47 & \cellcolor[HTML]{FDC877} 0.35 & \cellcolor[HTML]{FEF8B3} 0.48 & \cellcolor[HTML]{FEEC9F} 0.44 & \cellcolor[HTML]{FEF9B5} 0.48 & \cellcolor[HTML]{FDC675} 0.35 & \cellcolor[HTML]{E95739} 0.17 & \cellcolor[HTML]{F6814C} 0.23 & \cellcolor[HTML]{FDB668} 0.32 & \cellcolor[HTML]{CDE983} 0.62 & \cellcolor[HTML]{66BD63} 0.80 & \cellcolor[HTML]{E6F49D} 0.56 & \cellcolor[HTML]{FB9F5A} 0.28 & \cellcolor[HTML]{51B25D} 0.83 & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{158F4B} 0.91 & \cellcolor[HTML]{75C364} 0.78 & \cellcolor[HTML]{B3DE72} 0.67 & \cellcolor[HTML]{FEEA9D} 0.44 & \cellcolor[HTML]{FA9A58} 0.27 \\
tree\_200\_2 & Best & \cellcolor[HTML]{4BAF5C} 0.83 & \cellcolor[HTML]{7CC665} 0.76 & \cellcolor[HTML]{48AE5B} 0.84 & \cellcolor[HTML]{66BD63} 0.80 & \cellcolor[HTML]{60BA61} 0.81 & \cellcolor[HTML]{A2D769} 0.70 & \cellcolor[HTML]{2A9F54} 0.88 & \cellcolor[HTML]{19974F} 0.90 & \cellcolor[HTML]{F89053} 0.26 & \cellcolor[HTML]{F3FAAF} 0.53 & \cellcolor[HTML]{FEF8B3} 0.48 & \cellcolor[HTML]{C7E77F} 0.63 & \cellcolor[HTML]{8BCD67} 0.74 & \cellcolor[HTML]{9AD468} 0.72 & \cellcolor[HTML]{FEFBB9} 0.49 & \cellcolor[HTML]{FDB86A} 0.32 & \cellcolor[HTML]{FEE08B} 0.40 & \cellcolor[HTML]{FDBE6E} 0.33 & \cellcolor[HTML]{FEFAB7} 0.49 & \cellcolor[HTML]{F67C4A} 0.23 & \cellcolor[HTML]{98D268} 0.72 \\
tree\_200\_2 & Worst & \cellcolor[HTML]{B3DE72} 0.67 & \cellcolor[HTML]{C7E77F} 0.64 & \cellcolor[HTML]{FEF8B3} 0.48 & \cellcolor[HTML]{F2F9AD} 0.53 & \cellcolor[HTML]{E9F5A1} 0.56 & \cellcolor[HTML]{F2F9AD} 0.53 & \cellcolor[HTML]{FEE08B} 0.40 & \cellcolor[HTML]{F99354} 0.26 & \cellcolor[HTML]{FA9856} 0.27 & \cellcolor[HTML]{FEE391} 0.41 & \cellcolor[HTML]{D3EC87} 0.61 & \cellcolor[HTML]{CFEA84} 0.62 & \cellcolor[HTML]{C7E77F} 0.63 & \cellcolor[HTML]{F57948} 0.22 & \cellcolor[HTML]{9FD669} 0.71 & \cellcolor[HTML]{FDB668} 0.32 & \cellcolor[HTML]{8ECE67} 0.73 & \cellcolor[HTML]{FDC877} 0.35 & \cellcolor[HTML]{BDE278} 0.65 & \cellcolor[HTML]{F99354} 0.26 & \cellcolor[HTML]{FDBC6D} 0.33 \\
tree\_20\_0 & Best & \cellcolor[HTML]{016937} 0.99 & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{006837} 1.00 & \cellcolor[HTML]{138B49} 0.92 & \cellcolor[HTML]{A50026} 0.00 & \cellcolor[HTML]{FEE695} 0.42 & \cellcolor[HTML]{FEE18D} 0.41 & \cellcolor[HTML]{C7E77F} 0.63 & \cellcolor[HTML]{57B55F} 0.82 & \cellcolor[HTML]{BFE37A} 0.65 & \cellcolor[HTML]{60BA61} 0.81 & \cellcolor[HTML]{FDBE6E} 0.33 & \cellcolor[HTML]{51B25D} 0.83 & \cellcolor[HTML]{F7894F} 0.24 & \cellcolor[HTML]{F99354} 0.26 & \cellcolor[HTML]{FDC877} 0.35 & \cellcolor[HTML]{A4D869} 0.70 \\
tree\_20\_0 & Worst & \cellcolor[HTML]{E75236} 0.16 & \cellcolor[HTML]{FEE493} 0.41 & \cellcolor[HTML]{FDD884} 0.39 & \cellcolor[HTML]{95D168} 0.73 & \cellcolor[HTML]{FDBC6D} 0.33 & \cellcolor[HTML]{FEFEBD} 0.50 & \cellcolor[HTML]{FDDE89} 0.40 & \cellcolor[HTML]{F89053} 0.26 & \cellcolor[HTML]{E6F49D} 0.57 & \cellcolor[HTML]{E14631} 0.14 & \cellcolor[HTML]{C9E880} 0.63 & \cellcolor[HTML]{95D168} 0.73 & \cellcolor[HTML]{FEF3AB} 0.46 & \cellcolor[HTML]{E75236} 0.16 & \cellcolor[HTML]{FEF4AD} 0.47 & \cellcolor[HTML]{FDC877} 0.35 & \cellcolor[HTML]{FDC070} 0.34 & \cellcolor[HTML]{FEE493} 0.41 & \cellcolor[HTML]{BFE37A} 0.65 & \cellcolor[HTML]{F7834D} 0.24 & \cellcolor[HTML]{DF412F} 0.13 \\
tree\_50\_2 & Best & \cellcolor[HTML]{2A9F54} 0.88 & \cellcolor[HTML]{0B7C41} 0.95 & \cellcolor[HTML]{33A456} 0.86 & \cellcolor[HTML]{2A9F54} 0.88 & \cellcolor[HTML]{57B55F} 0.82 & \cellcolor[HTML]{70C164} 0.78 & \cellcolor[HTML]{118847} 0.93 & \cellcolor[HTML]{19974F} 0.90 & \cellcolor[HTML]{FEFBB9} 0.49 & \cellcolor[HTML]{FEEC9F} 0.44 & \cellcolor[HTML]{FEE18D} 0.41 & \cellcolor[HTML]{C7E77F} 0.63 & \cellcolor[HTML]{B3DE72} 0.67 & \cellcolor[HTML]{CDE983} 0.62 & \cellcolor[HTML]{98D268} 0.72 & \cellcolor[HTML]{FDC272} 0.34 & \cellcolor[HTML]{89CC66} 0.74 & \cellcolor[HTML]{FEF7B1} 0.48 & \cellcolor[HTML]{FEEEA3} 0.45 & \cellcolor[HTML]{FB9F5A} 0.28 & \cellcolor[HTML]{DAEF8D} 0.60 \\
tree\_50\_2 & Worst & \cellcolor[HTML]{FBFDB9} 0.51 & \cellcolor[HTML]{95D168} 0.73 & \cellcolor[HTML]{FDD884} 0.39 & \cellcolor[HTML]{ECF7A5} 0.55 & \cellcolor[HTML]{FDC070} 0.34 & \cellcolor[HTML]{FDDC87} 0.39 & \cellcolor[HTML]{FDAE61} 0.30 & \cellcolor[HTML]{D02926} 0.09 & \cellcolor[HTML]{E1F297} 0.57 & \cellcolor[HTML]{FCAA5F} 0.30 & \cellcolor[HTML]{DDF091} 0.59 & \cellcolor[HTML]{E6F49D} 0.56 & \cellcolor[HTML]{FEF9B5} 0.48 & \cellcolor[HTML]{D83328} 0.11 & \cellcolor[HTML]{75C364} 0.77 & \cellcolor[HTML]{FDBC6D} 0.33 & \cellcolor[HTML]{249D52} 0.88 & \cellcolor[HTML]{FEF8B3} 0.48 & \cellcolor[HTML]{54B45E} 0.82 & \cellcolor[HTML]{FEF1A7} 0.46 & \cellcolor[HTML]{ED5E3C} 0.18 \\
\bottomrule
\end{tabular}
\end{tiny}
\label{tab:my_label}
\end{table}


% \begin{table}

% \caption{[First results, not the final table]. The average values for 21 graph aesthetic measures for the 36 graphs (splitted into the judgements 'best' and 'worst) used in the evaluation. The values are normalised and higher values indicate higher quality. We calculated 21 measures, namely Node-Node Overlaps (\texttt{NNO}), the total area of Node-Node Overlaps (\texttt{NNOA}), Edge-Node Overlaps (\texttt{ENO}), the total area of Edge-Node Overlaps (\texttt{ENOA}), Node-Edge Overlaps (\texttt{NEO}), the total area of Node-Edge Overlaps (\texttt{NEOA}), the number of edge crossings (\texttt{CR}), stress (\texttt{ST}), crossing angular resolution (\texttt{CAR}), area (\texttt{AR}), aspect ratio (\texttt{ASP}), concentration (\texttt{CON}), node orthogonality (\texttt{NO}), Gabriel ratio (\texttt{GR}), angular resolution (\texttt{ANGR}), edge orthogonality (\texttt{EO}), edge length deviation (\texttt{ELD}), reflective edge symmetry (\texttt{ESR}), rotational edge symmetry (\texttt{ESO}), translational edge symmetry (\texttt{EST}), and the isometric projection measure (\texttt{ISO}).
% }
% \begin{tiny}
% \def\arraystretch{1.2}
% \setlength\tabcolsep{1pt}
% \begin{tabular}{llccccccccccccccccccccccc}
% \toprule
% graph & answer & NNO & NNOA & ENO & ENOA & NEO & NEOA & CR & ST & CAR & AR & ASP & CON & NO & GR & ANGR & EO & ELD & ESR & ESO & EST & ISO \\
% \midrule
% can\_24 & Best & \cellcolor[HTML]{083572} 0.98 & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{083E80} 0.95 & \cellcolor[HTML]{083978} 0.96 & \cellcolor[HTML]{083877} 0.97 & \cellcolor[HTML]{083B7B} 0.95 & \cellcolor[HTML]{083877} 0.97 & \cellcolor[HTML]{08488F} 0.90 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{6AADD5} 0.50 & \cellcolor[HTML]{BCD7EB} 0.28 & \cellcolor[HTML]{1764AB} 0.80 & \cellcolor[HTML]{0F5AA3} 0.84 & \cellcolor[HTML]{084388} 0.92 & \cellcolor[HTML]{1663AA} 0.80 & \cellcolor[HTML]{ACD0E6} 0.33 & \cellcolor[HTML]{1461A8} 0.81 & \cellcolor[HTML]{A7CEE4} 0.35 & \cellcolor[HTML]{B4D3E8} 0.31 & \cellcolor[HTML]{92C3DE} 0.40 & \cellcolor[HTML]{3D8DC3} 0.64 \\
% can\_24 & Worst & \cellcolor[HTML]{67ABD4} 0.51 & \cellcolor[HTML]{3484BF} 0.68 & \cellcolor[HTML]{97C6DF} 0.39 & \cellcolor[HTML]{519CCC} 0.57 & \cellcolor[HTML]{8BC0DD} 0.42 & \cellcolor[HTML]{63A9D3} 0.52 & \cellcolor[HTML]{DCE9F6} 0.14 & \cellcolor[HTML]{E4EEF8} 0.10 & \cellcolor[HTML]{D7E6F4} 0.16 & \cellcolor[HTML]{D6E5F4} 0.17 & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{6BAED6} 0.50 & \cellcolor[HTML]{85BCDB} 0.44 & \cellcolor[HTML]{DAE8F5} 0.14 & \cellcolor[HTML]{C3D9EE} 0.26 & \cellcolor[HTML]{8ABFDC} 0.42 & \cellcolor[HTML]{85BCDB} 0.43 & \cellcolor[HTML]{A0CAE1} 0.37 & \cellcolor[HTML]{6FB0D6} 0.49 & \cellcolor[HTML]{72B1D7} 0.48 & \cellcolor[HTML]{C5DAEE} 0.25 \\
% can\_96 & Best & \cellcolor[HTML]{084F99} 0.88 & \cellcolor[HTML]{083C7D} 0.95 & \cellcolor[HTML]{125EA6} 0.82 & \cellcolor[HTML]{125EA6} 0.82 & \cellcolor[HTML]{1967AD} 0.79 & \cellcolor[HTML]{1B6AAF} 0.78 & \cellcolor[HTML]{66AAD4} 0.51 & \cellcolor[HTML]{3383BE} 0.68 & \cellcolor[HTML]{4B98C9} 0.59 & \cellcolor[HTML]{A3CCE3} 0.36 & \cellcolor[HTML]{2272B5} 0.75 & \cellcolor[HTML]{3484BF} 0.67 & \cellcolor[HTML]{4F9BCB} 0.58 & \cellcolor[HTML]{1A68AE} 0.78 & \cellcolor[HTML]{82BADB} 0.44 & \cellcolor[HTML]{85BCDB} 0.44 & \cellcolor[HTML]{66AAD4} 0.51 & \cellcolor[HTML]{AACFE5} 0.34 & \cellcolor[HTML]{9AC7E0} 0.38 & \cellcolor[HTML]{6AADD5} 0.50 & \cellcolor[HTML]{4E9ACA} 0.59 \\
% can\_96 & Worst & \cellcolor[HTML]{3989C1} 0.66 & \cellcolor[HTML]{1764AB} 0.80 & \cellcolor[HTML]{2979B9} 0.72 & \cellcolor[HTML]{2777B8} 0.72 & \cellcolor[HTML]{2F7FBC} 0.69 & \cellcolor[HTML]{2A7AB9} 0.71 & \cellcolor[HTML]{A6CDE3} 0.35 & \cellcolor[HTML]{8ABFDC} 0.42 & \cellcolor[HTML]{3989C1} 0.66 & \cellcolor[HTML]{BED7EC} 0.28 & \cellcolor[HTML]{509BCB} 0.58 & \cellcolor[HTML]{3D8DC3} 0.64 & \cellcolor[HTML]{7BB7D9} 0.46 & \cellcolor[HTML]{3A8AC1} 0.66 & \cellcolor[HTML]{4A97C9} 0.60 & \cellcolor[HTML]{80B9DA} 0.45 & \cellcolor[HTML]{3A8AC1} 0.66 & \cellcolor[HTML]{A6CDE3} 0.35 & \cellcolor[HTML]{73B2D7} 0.48 & \cellcolor[HTML]{77B4D8} 0.47 & \cellcolor[HTML]{83BBDB} 0.44 \\
% dwt\_198 & Best & \cellcolor[HTML]{105CA4} 0.83 & \cellcolor[HTML]{1F6FB3} 0.76 & \cellcolor[HTML]{1764AB} 0.80 & \cellcolor[HTML]{1E6DB2} 0.77 & \cellcolor[HTML]{1461A8} 0.81 & \cellcolor[HTML]{1967AD} 0.79 & \cellcolor[HTML]{084E97} 0.89 & \cellcolor[HTML]{084B94} 0.89 & \cellcolor[HTML]{C5DAEE} 0.25 & \cellcolor[HTML]{AACFE5} 0.34 & \cellcolor[HTML]{B1D2E7} 0.31 & \cellcolor[HTML]{539DCC} 0.57 & \cellcolor[HTML]{6AADD5} 0.50 & \cellcolor[HTML]{1764AB} 0.80 & \cellcolor[HTML]{59A2CF} 0.55 & \cellcolor[HTML]{C3D9EE} 0.26 & \cellcolor[HTML]{4292C6} 0.62 & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{97C6DF} 0.39 & \cellcolor[HTML]{3B8BC2} 0.65 & \cellcolor[HTML]{70B1D7} 0.49 \\
% dwt\_198 & Worst & \cellcolor[HTML]{2F7FBC} 0.69 & \cellcolor[HTML]{3888C0} 0.66 & \cellcolor[HTML]{65AAD3} 0.52 & \cellcolor[HTML]{61A7D2} 0.53 & \cellcolor[HTML]{66AAD4} 0.52 & \cellcolor[HTML]{559FCD} 0.56 & \cellcolor[HTML]{77B4D8} 0.47 & \cellcolor[HTML]{1A69AE} 0.78 & \cellcolor[HTML]{9DC9E0} 0.38 & \cellcolor[HTML]{ADD0E6} 0.32 & \cellcolor[HTML]{AACFE5} 0.34 & \cellcolor[HTML]{6DAFD6} 0.49 & \cellcolor[HTML]{75B3D8} 0.48 & \cellcolor[HTML]{9DC9E0} 0.38 & \cellcolor[HTML]{1E6DB2} 0.76 & \cellcolor[HTML]{BCD7EB} 0.28 & \cellcolor[HTML]{63A9D3} 0.52 & \cellcolor[HTML]{5AA3CF} 0.55 & \cellcolor[HTML]{4F9BCB} 0.58 & \cellcolor[HTML]{3C8CC3} 0.65 & \cellcolor[HTML]{A3CCE3} 0.36 \\
% dwt\_209 & Best & \cellcolor[HTML]{08488F} 0.91 & \cellcolor[HTML]{084C96} 0.89 & \cellcolor[HTML]{0A549E} 0.86 & \cellcolor[HTML]{084C96} 0.89 & \cellcolor[HTML]{084A92} 0.90 & \cellcolor[HTML]{0A549E} 0.86 & \cellcolor[HTML]{0D58A1} 0.84 & \cellcolor[HTML]{084489} 0.92 & \cellcolor[HTML]{A0CAE1} 0.37 & \cellcolor[HTML]{4191C5} 0.63 & \cellcolor[HTML]{C5DAEE} 0.25 & \cellcolor[HTML]{3C8CC3} 0.65 & \cellcolor[HTML]{084F99} 0.88 & \cellcolor[HTML]{0C56A0} 0.85 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{66AAD4} 0.51 & \cellcolor[HTML]{4694C7} 0.61 & \cellcolor[HTML]{4795C8} 0.61 & \cellcolor[HTML]{4C99CA} 0.59 & \cellcolor[HTML]{4F9BCB} 0.58 & \cellcolor[HTML]{5CA3D0} 0.54 \\
% dwt\_209 & Worst & \cellcolor[HTML]{7BB7D9} 0.46 & \cellcolor[HTML]{5AA3CF} 0.55 & \cellcolor[HTML]{A6CDE3} 0.35 & \cellcolor[HTML]{509BCB} 0.58 & \cellcolor[HTML]{8FC1DD} 0.41 & \cellcolor[HTML]{58A1CE} 0.56 & \cellcolor[HTML]{D3E3F3} 0.18 & \cellcolor[HTML]{D7E6F4} 0.16 & \cellcolor[HTML]{C9DDF0} 0.23 & \cellcolor[HTML]{CEE0F1} 0.21 & \cellcolor[HTML]{1E6EB2} 0.76 & \cellcolor[HTML]{3989C1} 0.66 & \cellcolor[HTML]{6DAFD6} 0.49 & \cellcolor[HTML]{D1E2F2} 0.19 & \cellcolor[HTML]{A8CEE4} 0.34 & \cellcolor[HTML]{62A8D2} 0.53 & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{2474B6} 0.74 & \cellcolor[HTML]{0C56A0} 0.85 & \cellcolor[HTML]{08529C} 0.87 & \cellcolor[HTML]{D1E2F2} 0.19 \\
% grafo10183.100 & Best & \cellcolor[HTML]{105CA4} 0.83 & \cellcolor[HTML]{1562A9} 0.81 & \cellcolor[HTML]{08519C} 0.87 & \cellcolor[HTML]{1562A9} 0.81 & \cellcolor[HTML]{0F5AA3} 0.84 & \cellcolor[HTML]{1562A9} 0.81 & \cellcolor[HTML]{1461A8} 0.81 & \cellcolor[HTML]{1A69AE} 0.78 & \cellcolor[HTML]{9AC7E0} 0.38 & \cellcolor[HTML]{63A9D3} 0.52 & \cellcolor[HTML]{6FB0D6} 0.49 & \cellcolor[HTML]{2777B8} 0.72 & \cellcolor[HTML]{1E6DB2} 0.76 & \cellcolor[HTML]{3D8DC3} 0.64 & \cellcolor[HTML]{1E6DB2} 0.76 & \cellcolor[HTML]{A3CCE3} 0.36 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{B0D1E7} 0.32 & \cellcolor[HTML]{8BC0DD} 0.42 & \cellcolor[HTML]{A5CDE3} 0.35 & \cellcolor[HTML]{72B1D7} 0.48 \\
% grafo10183.100 & Worst & \cellcolor[HTML]{4B98C9} 0.59 & \cellcolor[HTML]{4292C6} 0.62 & \cellcolor[HTML]{3E8EC4} 0.64 & \cellcolor[HTML]{549ECD} 0.57 & \cellcolor[HTML]{3888C0} 0.66 & \cellcolor[HTML]{3181BD} 0.68 & \cellcolor[HTML]{83BBDB} 0.44 & \cellcolor[HTML]{C8DCEF} 0.24 & \cellcolor[HTML]{BBD6EB} 0.28 & \cellcolor[HTML]{92C3DE} 0.40 & \cellcolor[HTML]{61A7D2} 0.53 & \cellcolor[HTML]{2E7EBC} 0.70 & \cellcolor[HTML]{3B8BC2} 0.65 & \cellcolor[HTML]{CADDF0} 0.23 & \cellcolor[HTML]{90C2DE} 0.41 & \cellcolor[HTML]{98C7DF} 0.39 & \cellcolor[HTML]{A5CDE3} 0.35 & \cellcolor[HTML]{C1D9ED} 0.26 & \cellcolor[HTML]{4C99CA} 0.59 & \cellcolor[HTML]{ADD0E6} 0.32 & \cellcolor[HTML]{A2CBE2} 0.36 \\
% grafo2347.20 & Best & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{08316C} 0.99 & \cellcolor[HTML]{08336F} 0.99 & \cellcolor[HTML]{083C7D} 0.95 & \cellcolor[HTML]{084B94} 0.89 & \cellcolor[HTML]{B1D2E7} 0.32 & \cellcolor[HTML]{6BAED6} 0.50 & \cellcolor[HTML]{9BC8E0} 0.38 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{1F6FB3} 0.76 & \cellcolor[HTML]{084185} 0.93 & \cellcolor[HTML]{08519C} 0.87 & \cellcolor[HTML]{B0D1E7} 0.32 & \cellcolor[HTML]{08519C} 0.87 & \cellcolor[HTML]{ABCFE5} 0.33 & \cellcolor[HTML]{DAE8F5} 0.15 & \cellcolor[HTML]{C4DAEE} 0.26 & \cellcolor[HTML]{1B6AAF} 0.77 \\
% grafo2347.20 & Worst & \cellcolor[HTML]{B1D2E7} 0.31 & \cellcolor[HTML]{59A2CF} 0.55 & \cellcolor[HTML]{D1E2F2} 0.19 & \cellcolor[HTML]{6AADD5} 0.50 & \cellcolor[HTML]{A1CBE2} 0.37 & \cellcolor[HTML]{95C5DF} 0.40 & \cellcolor[HTML]{C6DBEF} 0.25 & \cellcolor[HTML]{DBE9F6} 0.14 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{BCD7EB} 0.28 & \cellcolor[HTML]{7AB6D9} 0.46 & \cellcolor[HTML]{87BDDC} 0.43 & \cellcolor[HTML]{5EA5D1} 0.54 & \cellcolor[HTML]{D3E3F3} 0.18 & \cellcolor[HTML]{AACFE5} 0.34 & \cellcolor[HTML]{8BC0DD} 0.42 & \cellcolor[HTML]{D4E4F3} 0.18 & \cellcolor[HTML]{1B6AAF} 0.77 & \cellcolor[HTML]{2F7FBC} 0.69 & \cellcolor[HTML]{6FB0D6} 0.49 & \cellcolor[HTML]{DBE9F6} 0.14 \\
% grafo5640.50 & Best & \cellcolor[HTML]{0F5BA3} 0.83 & \cellcolor[HTML]{08529C} 0.87 & \cellcolor[HTML]{0F5BA3} 0.84 & \cellcolor[HTML]{115DA5} 0.83 & \cellcolor[HTML]{2E7EBC} 0.70 & \cellcolor[HTML]{4090C5} 0.63 & \cellcolor[HTML]{0C57A0} 0.85 & \cellcolor[HTML]{0E59A2} 0.84 & \cellcolor[HTML]{C8DCEF} 0.24 & \cellcolor[HTML]{9AC7E0} 0.39 & \cellcolor[HTML]{92C3DE} 0.40 & \cellcolor[HTML]{2676B7} 0.73 & \cellcolor[HTML]{3A8AC1} 0.65 & \cellcolor[HTML]{519CCC} 0.57 & \cellcolor[HTML]{3C8CC3} 0.65 & \cellcolor[HTML]{A1CBE2} 0.37 & \cellcolor[HTML]{3A8AC1} 0.66 & \cellcolor[HTML]{B0D1E7} 0.32 & \cellcolor[HTML]{92C3DE} 0.41 & \cellcolor[HTML]{A8CEE4} 0.34 & \cellcolor[HTML]{3989C1} 0.66 \\
% grafo5640.50 & Worst & \cellcolor[HTML]{2C7CBB} 0.70 & \cellcolor[HTML]{1D6CB1} 0.77 & \cellcolor[HTML]{58A1CE} 0.56 & \cellcolor[HTML]{509BCB} 0.58 & \cellcolor[HTML]{62A8D2} 0.53 & \cellcolor[HTML]{60A6D1} 0.53 & \cellcolor[HTML]{82BADB} 0.44 & \cellcolor[HTML]{BAD6EA} 0.29 & \cellcolor[HTML]{C6DBEF} 0.25 & \cellcolor[HTML]{A0CAE1} 0.37 & \cellcolor[HTML]{72B1D7} 0.48 & \cellcolor[HTML]{2C7CBB} 0.70 & \cellcolor[HTML]{4896C8} 0.61 & \cellcolor[HTML]{CADDF0} 0.23 & \cellcolor[HTML]{105CA4} 0.83 & \cellcolor[HTML]{98C7DF} 0.39 & \cellcolor[HTML]{2E7EBC} 0.70 & \cellcolor[HTML]{85BCDB} 0.43 & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{77B4D8} 0.47 & \cellcolor[HTML]{77B4D8} 0.47 \\
% layered\_2\_20\_36 & Best & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{083877} 0.97 & \cellcolor[HTML]{083674} 0.97 & \cellcolor[HTML]{083A7A} 0.96 & \cellcolor[HTML]{083978} 0.96 & \cellcolor[HTML]{0C56A0} 0.85 & \cellcolor[HTML]{1A69AE} 0.78 & \cellcolor[HTML]{A7CEE4} 0.35 & \cellcolor[HTML]{8ABFDC} 0.42 & \cellcolor[HTML]{509BCB} 0.58 & \cellcolor[HTML]{1E6EB2} 0.76 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{5DA4D0} 0.54 & \cellcolor[HTML]{1C6BB0} 0.77 & \cellcolor[HTML]{75B3D8} 0.47 & \cellcolor[HTML]{4B98C9} 0.60 & \cellcolor[HTML]{AFD1E6} 0.32 & \cellcolor[HTML]{DCE9F6} 0.13 & \cellcolor[HTML]{CEE0F1} 0.21 & \cellcolor[HTML]{4594C7} 0.61 \\
% layered\_2\_20\_36 & Worst & \cellcolor[HTML]{2676B7} 0.73 & \cellcolor[HTML]{1A69AE} 0.78 & \cellcolor[HTML]{3B8BC2} 0.65 & \cellcolor[HTML]{2474B6} 0.74 & \cellcolor[HTML]{3B8BC2} 0.65 & \cellcolor[HTML]{2979B9} 0.72 & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{9DC9E0} 0.38 & \cellcolor[HTML]{B1D2E7} 0.32 & \cellcolor[HTML]{D0E1F2} 0.20 & \cellcolor[HTML]{4795C8} 0.61 & \cellcolor[HTML]{69ACD5} 0.51 & \cellcolor[HTML]{75B3D8} 0.48 & \cellcolor[HTML]{D1E2F2} 0.19 & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{6FB0D6} 0.49 & \cellcolor[HTML]{72B1D7} 0.48 & \cellcolor[HTML]{9DC9E0} 0.38 & \cellcolor[HTML]{BED7EC} 0.27 & \cellcolor[HTML]{AFD1E6} 0.32 & \cellcolor[HTML]{CDDFF1} 0.21 \\
% layered\_2\_20\_38 & Best & \cellcolor[HTML]{083674} 0.98 & \cellcolor[HTML]{08316C} 0.99 & \cellcolor[HTML]{083F82} 0.94 & \cellcolor[HTML]{083877} 0.97 & \cellcolor[HTML]{084489} 0.92 & \cellcolor[HTML]{08458B} 0.92 & \cellcolor[HTML]{0C56A0} 0.85 & \cellcolor[HTML]{115DA5} 0.82 & \cellcolor[HTML]{98C7DF} 0.39 & \cellcolor[HTML]{63A9D3} 0.52 & \cellcolor[HTML]{549ECD} 0.57 & \cellcolor[HTML]{1E6EB2} 0.76 & \cellcolor[HTML]{1562A9} 0.81 & \cellcolor[HTML]{70B1D7} 0.49 & \cellcolor[HTML]{2070B4} 0.75 & \cellcolor[HTML]{83BBDB} 0.44 & \cellcolor[HTML]{62A8D2} 0.52 & \cellcolor[HTML]{A0CAE1} 0.37 & \cellcolor[HTML]{C1D9ED} 0.26 & \cellcolor[HTML]{BAD6EA} 0.29 & \cellcolor[HTML]{3989C1} 0.66 \\
% layered\_2\_20\_38 & Worst & \cellcolor[HTML]{2A7AB9} 0.71 & \cellcolor[HTML]{2070B4} 0.75 & \cellcolor[HTML]{3D8DC3} 0.64 & \cellcolor[HTML]{2777B8} 0.73 & \cellcolor[HTML]{4594C7} 0.62 & \cellcolor[HTML]{4090C5} 0.63 & \cellcolor[HTML]{4292C6} 0.62 & \cellcolor[HTML]{4694C7} 0.61 & \cellcolor[HTML]{A6CDE3} 0.35 & \cellcolor[HTML]{BCD7EB} 0.28 & \cellcolor[HTML]{7FB8DA} 0.45 & \cellcolor[HTML]{4F9BCB} 0.58 & \cellcolor[HTML]{60A6D1} 0.53 & \cellcolor[HTML]{B4D3E8} 0.31 & \cellcolor[HTML]{66AAD4} 0.51 & \cellcolor[HTML]{83BBDB} 0.44 & \cellcolor[HTML]{3F8FC4} 0.63 & \cellcolor[HTML]{8DC0DD} 0.42 & \cellcolor[HTML]{ACD0E6} 0.33 & \cellcolor[HTML]{72B1D7} 0.48 & \cellcolor[HTML]{A8CEE4} 0.34 \\
% layered\_2\_20\_40 & Best & \cellcolor[HTML]{08326E} 0.99 & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{084286} 0.93 & \cellcolor[HTML]{083C7D} 0.95 & \cellcolor[HTML]{08488F} 0.90 & \cellcolor[HTML]{084388} 0.93 & \cellcolor[HTML]{3B8BC2} 0.65 & \cellcolor[HTML]{4191C5} 0.63 & \cellcolor[HTML]{6DAFD6} 0.49 & \cellcolor[HTML]{8BC0DD} 0.42 & \cellcolor[HTML]{3C8CC3} 0.65 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{3383BE} 0.68 & \cellcolor[HTML]{61A7D2} 0.53 & \cellcolor[HTML]{1B6AAF} 0.78 & \cellcolor[HTML]{A6CDE3} 0.35 & \cellcolor[HTML]{85BCDB} 0.43 & \cellcolor[HTML]{97C6DF} 0.39 & \cellcolor[HTML]{C1D9ED} 0.26 & \cellcolor[HTML]{CDDFF1} 0.21 & \cellcolor[HTML]{6FB0D6} 0.49 \\
% layered\_2\_20\_40 & Worst & \cellcolor[HTML]{1866AC} 0.79 & \cellcolor[HTML]{0D58A1} 0.84 & \cellcolor[HTML]{3C8CC3} 0.65 & \cellcolor[HTML]{3F8FC4} 0.64 & \cellcolor[HTML]{58A1CE} 0.56 & \cellcolor[HTML]{4292C6} 0.62 & \cellcolor[HTML]{509BCB} 0.58 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{70B1D7} 0.48 & \cellcolor[HTML]{A1CBE2} 0.36 & \cellcolor[HTML]{549ECD} 0.57 & \cellcolor[HTML]{3989C1} 0.66 & \cellcolor[HTML]{4292C6} 0.62 & \cellcolor[HTML]{88BEDC} 0.43 & \cellcolor[HTML]{5DA4D0} 0.54 & \cellcolor[HTML]{97C6DF} 0.39 & \cellcolor[HTML]{65AAD3} 0.52 & \cellcolor[HTML]{82BADB} 0.44 & \cellcolor[HTML]{C0D8ED} 0.27 & \cellcolor[HTML]{9ECAE1} 0.37 & \cellcolor[HTML]{85BCDB} 0.44 \\
% layered\_2\_50\_101 & Best & \cellcolor[HTML]{083E80} 0.94 & \cellcolor[HTML]{083674} 0.97 & \cellcolor[HTML]{084A92} 0.90 & \cellcolor[HTML]{084489} 0.92 & \cellcolor[HTML]{084991} 0.90 & \cellcolor[HTML]{084B94} 0.89 & \cellcolor[HTML]{2878B8} 0.72 & \cellcolor[HTML]{61A7D2} 0.53 & \cellcolor[HTML]{4F9BCB} 0.59 & \cellcolor[HTML]{87BDDC} 0.43 & \cellcolor[HTML]{63A9D3} 0.52 & \cellcolor[HTML]{2979B9} 0.72 & \cellcolor[HTML]{3585BF} 0.67 & \cellcolor[HTML]{559FCD} 0.56 & \cellcolor[HTML]{125EA6} 0.82 & \cellcolor[HTML]{9DC9E0} 0.38 & \cellcolor[HTML]{A2CBE2} 0.36 & \cellcolor[HTML]{87BDDC} 0.43 & \cellcolor[HTML]{9AC7E0} 0.39 & \cellcolor[HTML]{B0D1E7} 0.32 & \cellcolor[HTML]{5DA4D0} 0.54 \\
% layered\_2\_50\_101 & Worst & \cellcolor[HTML]{1967AD} 0.79 & \cellcolor[HTML]{0F5BA3} 0.83 & \cellcolor[HTML]{1B6AAF} 0.78 & \cellcolor[HTML]{1866AC} 0.79 & \cellcolor[HTML]{2C7CBB} 0.71 & \cellcolor[HTML]{2575B7} 0.73 & \cellcolor[HTML]{2A7AB9} 0.71 & \cellcolor[HTML]{2C7CBB} 0.71 & \cellcolor[HTML]{82BADB} 0.44 & \cellcolor[HTML]{AACFE5} 0.34 & \cellcolor[HTML]{97C6DF} 0.39 & \cellcolor[HTML]{3282BE} 0.68 & \cellcolor[HTML]{519CCC} 0.58 & \cellcolor[HTML]{3383BE} 0.68 & \cellcolor[HTML]{2373B6} 0.74 & \cellcolor[HTML]{7AB6D9} 0.46 & \cellcolor[HTML]{2979B9} 0.72 & \cellcolor[HTML]{ABCFE5} 0.33 & \cellcolor[HTML]{9DC9E0} 0.38 & \cellcolor[HTML]{9BC8E0} 0.38 & \cellcolor[HTML]{CBDEF0} 0.23 \\
% layered\_2\_50\_102 & Best & \cellcolor[HTML]{083A7A} 0.96 & \cellcolor[HTML]{083471} 0.98 & \cellcolor[HTML]{084A92} 0.90 & \cellcolor[HTML]{083F82} 0.94 & \cellcolor[HTML]{08478E} 0.91 & \cellcolor[HTML]{08468C} 0.91 & \cellcolor[HTML]{3080BD} 0.69 & \cellcolor[HTML]{83BBDB} 0.44 & \cellcolor[HTML]{66AAD4} 0.51 & \cellcolor[HTML]{95C5DF} 0.40 & \cellcolor[HTML]{3787C0} 0.67 & \cellcolor[HTML]{1663AA} 0.80 & \cellcolor[HTML]{2979B9} 0.72 & \cellcolor[HTML]{4F9BCB} 0.59 & \cellcolor[HTML]{2373B6} 0.74 & \cellcolor[HTML]{D0E1F2} 0.20 & \cellcolor[HTML]{98C7DF} 0.39 & \cellcolor[HTML]{72B1D7} 0.48 & \cellcolor[HTML]{66AAD4} 0.51 & \cellcolor[HTML]{AFD1E6} 0.32 & \cellcolor[HTML]{6DAFD6} 0.50 \\
% layered\_2\_50\_102 & Worst & \cellcolor[HTML]{2474B6} 0.74 & \cellcolor[HTML]{1E6DB2} 0.76 & \cellcolor[HTML]{3A8AC1} 0.66 & \cellcolor[HTML]{2B7BBA} 0.71 & \cellcolor[HTML]{4A97C9} 0.60 & \cellcolor[HTML]{4191C5} 0.63 & \cellcolor[HTML]{3484BF} 0.67 & \cellcolor[HTML]{5DA4D0} 0.54 & \cellcolor[HTML]{83BBDB} 0.44 & \cellcolor[HTML]{A3CCE3} 0.36 & \cellcolor[HTML]{3A8AC1} 0.66 & \cellcolor[HTML]{2B7BBA} 0.71 & \cellcolor[HTML]{3787C0} 0.67 & \cellcolor[HTML]{61A7D2} 0.53 & \cellcolor[HTML]{4F9BCB} 0.58 & \cellcolor[HTML]{C8DCEF} 0.24 & \cellcolor[HTML]{59A2CF} 0.55 & \cellcolor[HTML]{7AB6D9} 0.46 & \cellcolor[HTML]{63A9D3} 0.52 & \cellcolor[HTML]{7BB7D9} 0.46 & \cellcolor[HTML]{75B3D8} 0.47 \\
% layered\_2\_50\_93 & Best & \cellcolor[HTML]{083674} 0.98 & \cellcolor[HTML]{08316C} 0.99 & \cellcolor[HTML]{084185} 0.93 & \cellcolor[HTML]{084185} 0.93 & \cellcolor[HTML]{083F82} 0.94 & \cellcolor[HTML]{08458B} 0.92 & \cellcolor[HTML]{3C8CC3} 0.65 & \cellcolor[HTML]{5DA4D0} 0.54 & \cellcolor[HTML]{2D7DBB} 0.70 & \cellcolor[HTML]{9DC9E0} 0.38 & \cellcolor[HTML]{5CA3D0} 0.54 & \cellcolor[HTML]{135FA7} 0.82 & \cellcolor[HTML]{4292C6} 0.62 & \cellcolor[HTML]{4A97C9} 0.60 & \cellcolor[HTML]{1461A8} 0.81 & \cellcolor[HTML]{72B1D7} 0.48 & \cellcolor[HTML]{9BC8E0} 0.38 & \cellcolor[HTML]{509BCB} 0.58 & \cellcolor[HTML]{B5D3E9} 0.30 & \cellcolor[HTML]{C7DBEF} 0.24 & \cellcolor[HTML]{BBD6EB} 0.28 \\
% layered\_2\_50\_93 & Worst & \cellcolor[HTML]{2B7BBA} 0.71 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{2F7FBC} 0.69 & \cellcolor[HTML]{2A7AB9} 0.71 & \cellcolor[HTML]{2D7DBB} 0.70 & \cellcolor[HTML]{2A7AB9} 0.71 & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{4292C6} 0.62 & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{B6D4E9} 0.30 & \cellcolor[HTML]{A7CEE4} 0.34 & \cellcolor[HTML]{3787C0} 0.67 & \cellcolor[HTML]{58A1CE} 0.56 & \cellcolor[HTML]{5EA5D1} 0.54 & \cellcolor[HTML]{3383BE} 0.68 & \cellcolor[HTML]{73B2D7} 0.48 & \cellcolor[HTML]{3F8FC4} 0.64 & \cellcolor[HTML]{3E8EC4} 0.64 & \cellcolor[HTML]{B1D2E7} 0.31 & \cellcolor[HTML]{9AC7E0} 0.38 & \cellcolor[HTML]{A5CDE3} 0.35 \\
% layered\_3\_100\_207 & Best & \cellcolor[HTML]{0D58A1} 0.85 & \cellcolor[HTML]{084B94} 0.89 & \cellcolor[HTML]{0B559F} 0.86 & \cellcolor[HTML]{0C57A0} 0.85 & \cellcolor[HTML]{0D58A1} 0.85 & \cellcolor[HTML]{1D6CB1} 0.77 & \cellcolor[HTML]{1E6EB2} 0.76 & \cellcolor[HTML]{1D6CB1} 0.77 & \cellcolor[HTML]{E1EDF8} 0.11 & \cellcolor[HTML]{93C4DE} 0.40 & \cellcolor[HTML]{5AA3CF} 0.55 & \cellcolor[HTML]{2878B8} 0.72 & \cellcolor[HTML]{4A97C9} 0.60 & \cellcolor[HTML]{66AAD4} 0.51 & \cellcolor[HTML]{1A69AE} 0.78 & \cellcolor[HTML]{BFD8EC} 0.27 & \cellcolor[HTML]{C3D9EE} 0.26 & \cellcolor[HTML]{3989C1} 0.66 & \cellcolor[HTML]{4795C8} 0.61 & \cellcolor[HTML]{D1E2F2} 0.19 & \cellcolor[HTML]{70B1D7} 0.49 \\
% layered\_3\_100\_207 & Worst & \cellcolor[HTML]{1C6BB0} 0.77 & \cellcolor[HTML]{1866AC} 0.79 & \cellcolor[HTML]{3080BD} 0.69 & \cellcolor[HTML]{3181BD} 0.68 & \cellcolor[HTML]{2F7FBC} 0.69 & \cellcolor[HTML]{3F8FC4} 0.63 & \cellcolor[HTML]{CFE1F2} 0.20 & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{E7F0F9} 0.08 & \cellcolor[HTML]{C7DBEF} 0.25 & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{0F5BA3} 0.83 & \cellcolor[HTML]{8BC0DD} 0.42 & \cellcolor[HTML]{D2E3F3} 0.19 & \cellcolor[HTML]{084C96} 0.89 & \cellcolor[HTML]{CBDEF0} 0.22 & \cellcolor[HTML]{0C56A0} 0.85 & \cellcolor[HTML]{3F8FC4} 0.64 & \cellcolor[HTML]{2A7AB9} 0.71 & \cellcolor[HTML]{C1D9ED} 0.26 & \cellcolor[HTML]{D3E3F3} 0.18 \\
% layered\_3\_100\_253 & Best & \cellcolor[HTML]{0B559F} 0.86 & \cellcolor[HTML]{084489} 0.92 & \cellcolor[HTML]{084F99} 0.88 & \cellcolor[HTML]{08509A} 0.88 & \cellcolor[HTML]{0A549E} 0.86 & \cellcolor[HTML]{0B559F} 0.86 & \cellcolor[HTML]{4191C5} 0.63 & \cellcolor[HTML]{3A8AC1} 0.66 & \cellcolor[HTML]{2D7DBB} 0.70 & \cellcolor[HTML]{83BBDB} 0.44 & \cellcolor[HTML]{2676B7} 0.73 & \cellcolor[HTML]{2070B4} 0.75 & \cellcolor[HTML]{3484BF} 0.67 & \cellcolor[HTML]{3C8CC3} 0.65 & \cellcolor[HTML]{1764AB} 0.80 & \cellcolor[HTML]{D5E5F4} 0.17 & \cellcolor[HTML]{B1D2E7} 0.31 & \cellcolor[HTML]{DBE9F6} 0.14 & \cellcolor[HTML]{9DC9E0} 0.38 & \cellcolor[HTML]{D8E7F5} 0.15 & \cellcolor[HTML]{57A0CE} 0.56 \\
% layered\_3\_100\_253 & Worst & \cellcolor[HTML]{1562A9} 0.80 & \cellcolor[HTML]{08529C} 0.87 & \cellcolor[HTML]{3282BE} 0.68 & \cellcolor[HTML]{2676B7} 0.73 & \cellcolor[HTML]{3787C0} 0.66 & \cellcolor[HTML]{2C7CBB} 0.70 & \cellcolor[HTML]{BED7EC} 0.28 & \cellcolor[HTML]{CBDEF0} 0.22 & \cellcolor[HTML]{519CCC} 0.58 & \cellcolor[HTML]{AFD1E6} 0.32 & \cellcolor[HTML]{72B1D7} 0.48 & \cellcolor[HTML]{0F5AA3} 0.84 & \cellcolor[HTML]{5EA5D1} 0.54 & \cellcolor[HTML]{D5E5F4} 0.17 & \cellcolor[HTML]{084B94} 0.89 & \cellcolor[HTML]{D5E5F4} 0.17 & \cellcolor[HTML]{1967AD} 0.79 & \cellcolor[HTML]{D7E6F4} 0.16 & \cellcolor[HTML]{6DAFD6} 0.49 & \cellcolor[HTML]{C7DBEF} 0.24 & \cellcolor[HTML]{C9DDF0} 0.23 \\
% layered\_3\_100\_284 & Best & \cellcolor[HTML]{0A549E} 0.86 & \cellcolor[HTML]{08458B} 0.92 & \cellcolor[HTML]{084286} 0.93 & \cellcolor[HTML]{09539D} 0.86 & \cellcolor[HTML]{0B559F} 0.86 & \cellcolor[HTML]{0E59A2} 0.84 & \cellcolor[HTML]{0B559F} 0.86 & \cellcolor[HTML]{084A92} 0.90 & \cellcolor[HTML]{ADD0E6} 0.32 & \cellcolor[HTML]{4B98C9} 0.60 & \cellcolor[HTML]{3484BF} 0.67 & \cellcolor[HTML]{3888C0} 0.66 & \cellcolor[HTML]{1866AC} 0.79 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{3282BE} 0.68 & \cellcolor[HTML]{70B1D7} 0.49 & \cellcolor[HTML]{D2E3F3} 0.18 & \cellcolor[HTML]{2474B6} 0.73 & \cellcolor[HTML]{98C7DF} 0.39 & \cellcolor[HTML]{9AC7E0} 0.38 & \cellcolor[HTML]{519CCC} 0.58 \\
% layered\_3\_100\_284 & Worst & \cellcolor[HTML]{2373B6} 0.74 & \cellcolor[HTML]{1663AA} 0.80 & \cellcolor[HTML]{3080BD} 0.69 & \cellcolor[HTML]{3888C0} 0.66 & \cellcolor[HTML]{3888C0} 0.66 & \cellcolor[HTML]{2B7BBA} 0.71 & \cellcolor[HTML]{B9D5EA} 0.29 & \cellcolor[HTML]{ACD0E6} 0.33 & \cellcolor[HTML]{85BCDB} 0.44 & \cellcolor[HTML]{72B1D7} 0.48 & \cellcolor[HTML]{73B2D7} 0.48 & \cellcolor[HTML]{2E7EBC} 0.70 & \cellcolor[HTML]{3080BD} 0.69 & \cellcolor[HTML]{D8E7F5} 0.15 & \cellcolor[HTML]{3181BD} 0.68 & \cellcolor[HTML]{73B2D7} 0.48 & \cellcolor[HTML]{1E6EB2} 0.76 & \cellcolor[HTML]{2373B6} 0.74 & \cellcolor[HTML]{5DA4D0} 0.54 & \cellcolor[HTML]{5EA5D1} 0.54 & \cellcolor[HTML]{D0E1F2} 0.20 \\
% layered\_3\_200\_431 & Best & \cellcolor[HTML]{084A92} 0.90 & \cellcolor[HTML]{08458B} 0.92 & \cellcolor[HTML]{08529C} 0.87 & \cellcolor[HTML]{0E59A2} 0.84 & \cellcolor[HTML]{084E97} 0.89 & \cellcolor[HTML]{125EA6} 0.82 & \cellcolor[HTML]{1360A7} 0.81 & \cellcolor[HTML]{1A69AE} 0.78 & \cellcolor[HTML]{ACD0E6} 0.33 & \cellcolor[HTML]{70B1D7} 0.48 & \cellcolor[HTML]{5EA5D1} 0.54 & \cellcolor[HTML]{2474B6} 0.74 & \cellcolor[HTML]{3282BE} 0.68 & \cellcolor[HTML]{2E7EBC} 0.70 & \cellcolor[HTML]{0B559F} 0.86 & \cellcolor[HTML]{BED7EC} 0.27 & \cellcolor[HTML]{B7D4EA} 0.30 & \cellcolor[HTML]{E8F1FA} 0.07 & \cellcolor[HTML]{C9DDF0} 0.23 & \cellcolor[HTML]{BED7EC} 0.28 & \cellcolor[HTML]{3383BE} 0.68 \\
% layered\_3\_200\_431 & Worst & \cellcolor[HTML]{08509A} 0.88 & \cellcolor[HTML]{08509A} 0.88 & \cellcolor[HTML]{3383BE} 0.68 & \cellcolor[HTML]{4694C7} 0.61 & \cellcolor[HTML]{1866AC} 0.79 & \cellcolor[HTML]{2979B9} 0.72 & \cellcolor[HTML]{D4E4F3} 0.18 & \cellcolor[HTML]{A6CDE3} 0.35 & \cellcolor[HTML]{6AADD5} 0.50 & \cellcolor[HTML]{A2CBE2} 0.36 & \cellcolor[HTML]{A0CAE1} 0.37 & \cellcolor[HTML]{1360A7} 0.82 & \cellcolor[HTML]{559FCD} 0.56 & \cellcolor[HTML]{D9E7F5} 0.15 & \cellcolor[HTML]{084B94} 0.89 & \cellcolor[HTML]{B4D3E8} 0.31 & \cellcolor[HTML]{08519C} 0.87 & \cellcolor[HTML]{E8F1FA} 0.07 & \cellcolor[HTML]{ABCFE5} 0.34 & \cellcolor[HTML]{92C3DE} 0.40 & \cellcolor[HTML]{DDEAF6} 0.13 \\
% layered\_3\_200\_487 & Best & \cellcolor[HTML]{1461A8} 0.81 & \cellcolor[HTML]{09539D} 0.86 & \cellcolor[HTML]{1360A7} 0.82 & \cellcolor[HTML]{0D58A1} 0.84 & \cellcolor[HTML]{1360A7} 0.81 & \cellcolor[HTML]{1764AB} 0.80 & \cellcolor[HTML]{084F99} 0.88 & \cellcolor[HTML]{2777B8} 0.73 & \cellcolor[HTML]{5AA3CF} 0.55 & \cellcolor[HTML]{70B1D7} 0.49 & \cellcolor[HTML]{3F8FC4} 0.64 & \cellcolor[HTML]{4B98C9} 0.59 & \cellcolor[HTML]{2676B7} 0.73 & \cellcolor[HTML]{2474B6} 0.74 & \cellcolor[HTML]{2979B9} 0.72 & \cellcolor[HTML]{A0CAE1} 0.37 & \cellcolor[HTML]{CDDFF1} 0.21 & \cellcolor[HTML]{135FA7} 0.82 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{C8DCEF} 0.24 & \cellcolor[HTML]{5AA3CF} 0.55 \\
% layered\_3\_200\_487 & Worst & \cellcolor[HTML]{0F5AA3} 0.84 & \cellcolor[HTML]{0D58A1} 0.85 & \cellcolor[HTML]{4C99CA} 0.59 & \cellcolor[HTML]{3D8DC3} 0.64 & \cellcolor[HTML]{4090C5} 0.63 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{B0D1E7} 0.32 & \cellcolor[HTML]{85BCDB} 0.43 & \cellcolor[HTML]{1A69AE} 0.78 & \cellcolor[HTML]{BED7EC} 0.27 & \cellcolor[HTML]{85BCDB} 0.44 & \cellcolor[HTML]{1E6DB2} 0.76 & \cellcolor[HTML]{62A8D2} 0.53 & \cellcolor[HTML]{C8DCEF} 0.24 & \cellcolor[HTML]{0C56A0} 0.85 & \cellcolor[HTML]{A0CAE1} 0.37 & \cellcolor[HTML]{1764AB} 0.80 & \cellcolor[HTML]{084C96} 0.89 & \cellcolor[HTML]{135FA7} 0.82 & \cellcolor[HTML]{A1CBE2} 0.36 & \cellcolor[HTML]{CADDF0} 0.23 \\
% layered\_3\_200\_508 & Best & \cellcolor[HTML]{1D6CB1} 0.77 & \cellcolor[HTML]{0F5BA3} 0.83 & \cellcolor[HTML]{08519C} 0.87 & \cellcolor[HTML]{135FA7} 0.82 & \cellcolor[HTML]{1562A9} 0.81 & \cellcolor[HTML]{135FA7} 0.82 & \cellcolor[HTML]{0A549E} 0.86 & \cellcolor[HTML]{0D58A1} 0.84 & \cellcolor[HTML]{75B3D8} 0.48 & \cellcolor[HTML]{8BC0DD} 0.42 & \cellcolor[HTML]{62A8D2} 0.52 & \cellcolor[HTML]{4A97C9} 0.60 & \cellcolor[HTML]{3181BD} 0.69 & \cellcolor[HTML]{559FCD} 0.57 & \cellcolor[HTML]{1F6FB3} 0.76 & \cellcolor[HTML]{8DC0DD} 0.42 & \cellcolor[HTML]{D1E2F2} 0.19 & \cellcolor[HTML]{E2EDF8} 0.10 & \cellcolor[HTML]{4A97C9} 0.60 & \cellcolor[HTML]{6DAFD6} 0.49 & \cellcolor[HTML]{4795C8} 0.61 \\
% layered\_3\_200\_508 & Worst & \cellcolor[HTML]{0C56A0} 0.85 & \cellcolor[HTML]{0B559F} 0.86 & \cellcolor[HTML]{2070B4} 0.75 & \cellcolor[HTML]{2D7DBB} 0.70 & \cellcolor[HTML]{4B98C9} 0.60 & \cellcolor[HTML]{3F8FC4} 0.64 & \cellcolor[HTML]{B2D2E8} 0.31 & \cellcolor[HTML]{A8CEE4} 0.34 & \cellcolor[HTML]{509BCB} 0.58 & \cellcolor[HTML]{B6D4E9} 0.30 & \cellcolor[HTML]{59A2CF} 0.55 & \cellcolor[HTML]{1866AC} 0.79 & \cellcolor[HTML]{4F9BCB} 0.58 & \cellcolor[HTML]{E9F2FA} 0.07 & \cellcolor[HTML]{08488F} 0.90 & \cellcolor[HTML]{88BEDC} 0.43 & \cellcolor[HTML]{084C96} 0.89 & \cellcolor[HTML]{E3EEF8} 0.10 & \cellcolor[HTML]{2878B8} 0.72 & \cellcolor[HTML]{66AAD4} 0.51 & \cellcolor[HTML]{C7DBEF} 0.24 \\
% mesh1em1 & Best & \cellcolor[HTML]{084A92} 0.90 & \cellcolor[HTML]{084286} 0.93 & \cellcolor[HTML]{084C96} 0.89 & \cellcolor[HTML]{08529C} 0.87 & \cellcolor[HTML]{084F99} 0.88 & \cellcolor[HTML]{09539D} 0.87 & \cellcolor[HTML]{125EA6} 0.82 & \cellcolor[HTML]{2676B7} 0.73 & \cellcolor[HTML]{3C8CC3} 0.64 & \cellcolor[HTML]{82BADB} 0.44 & \cellcolor[HTML]{62A8D2} 0.52 & \cellcolor[HTML]{1562A9} 0.81 & \cellcolor[HTML]{4594C7} 0.61 & \cellcolor[HTML]{1D6CB1} 0.77 & \cellcolor[HTML]{2D7DBB} 0.70 & \cellcolor[HTML]{A0CAE1} 0.37 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{2F7FBC} 0.69 & \cellcolor[HTML]{58A1CE} 0.56 & \cellcolor[HTML]{8ABFDC} 0.42 & \cellcolor[HTML]{B0D1E7} 0.32 \\
% mesh1em1 & Worst & \cellcolor[HTML]{2D7DBB} 0.70 & \cellcolor[HTML]{1C6BB0} 0.77 & \cellcolor[HTML]{3888C0} 0.66 & \cellcolor[HTML]{3C8CC3} 0.64 & \cellcolor[HTML]{559FCD} 0.57 & \cellcolor[HTML]{3F8FC4} 0.64 & \cellcolor[HTML]{5AA3CF} 0.55 & \cellcolor[HTML]{82BADB} 0.44 & \cellcolor[HTML]{9ECAE1} 0.37 & \cellcolor[HTML]{BCD7EB} 0.28 & \cellcolor[HTML]{4896C8} 0.60 & \cellcolor[HTML]{4E9ACA} 0.59 & \cellcolor[HTML]{82BADB} 0.44 & \cellcolor[HTML]{90C2DE} 0.41 & \cellcolor[HTML]{88BEDC} 0.43 & \cellcolor[HTML]{9ECAE1} 0.37 & \cellcolor[HTML]{8FC1DD} 0.41 & \cellcolor[HTML]{2A7AB9} 0.71 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{80B9DA} 0.45 & \cellcolor[HTML]{6FB0D6} 0.49 \\
% sem\_0\_20\_16 & Best & \cellcolor[HTML]{084388} 0.92 & \cellcolor[HTML]{083D7E} 0.95 & \cellcolor[HTML]{083978} 0.96 & \cellcolor[HTML]{083978} 0.96 & \cellcolor[HTML]{084E97} 0.88 & \cellcolor[HTML]{0A549E} 0.86 & \cellcolor[HTML]{2272B5} 0.74 & \cellcolor[HTML]{1D6CB1} 0.77 & \cellcolor[HTML]{2272B5} 0.74 & \cellcolor[HTML]{66AAD4} 0.51 & \cellcolor[HTML]{559FCD} 0.56 & \cellcolor[HTML]{1A68AE} 0.78 & \cellcolor[HTML]{1461A8} 0.81 & \cellcolor[HTML]{3E8EC4} 0.64 & \cellcolor[HTML]{3787C0} 0.67 & \cellcolor[HTML]{B0D1E7} 0.32 & \cellcolor[HTML]{1E6EB2} 0.76 & \cellcolor[HTML]{B0D1E7} 0.32 & \cellcolor[HTML]{B9D5EA} 0.29 & \cellcolor[HTML]{E4EFF9} 0.09 & \cellcolor[HTML]{7DB8D9} 0.46 \\
% sem\_0\_20\_16 & Worst & \cellcolor[HTML]{3484BF} 0.67 & \cellcolor[HTML]{2B7BBA} 0.71 & \cellcolor[HTML]{2A7AB9} 0.71 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{4594C7} 0.62 & \cellcolor[HTML]{6FB0D6} 0.49 & \cellcolor[HTML]{1C6BB0} 0.77 & \cellcolor[HTML]{97C6DF} 0.39 & \cellcolor[HTML]{7BB7D9} 0.46 & \cellcolor[HTML]{C1D9ED} 0.26 & \cellcolor[HTML]{A0CAE1} 0.37 & \cellcolor[HTML]{6FB0D6} 0.49 & \cellcolor[HTML]{62A8D2} 0.52 & \cellcolor[HTML]{BCD7EB} 0.28 & \cellcolor[HTML]{3383BE} 0.68 & \cellcolor[HTML]{A0CAE1} 0.37 & \cellcolor[HTML]{5EA5D1} 0.54 & \cellcolor[HTML]{D2E3F3} 0.18 & \cellcolor[HTML]{B4D3E8} 0.31 & \cellcolor[HTML]{CFE1F2} 0.20 & \cellcolor[HTML]{A8CEE4} 0.34 \\
% sem\_0\_50\_100 & Best & \cellcolor[HTML]{084489} 0.92 & \cellcolor[HTML]{084C96} 0.89 & \cellcolor[HTML]{084083} 0.93 & \cellcolor[HTML]{084991} 0.90 & \cellcolor[HTML]{08478E} 0.91 & \cellcolor[HTML]{08478E} 0.91 & \cellcolor[HTML]{115DA5} 0.83 & \cellcolor[HTML]{135FA7} 0.82 & \cellcolor[HTML]{6BAED6} 0.50 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{3585BF} 0.67 & \cellcolor[HTML]{125EA6} 0.82 & \cellcolor[HTML]{08458B} 0.92 & \cellcolor[HTML]{2F7FBC} 0.69 & \cellcolor[HTML]{1B6AAF} 0.78 & \cellcolor[HTML]{72B1D7} 0.48 & \cellcolor[HTML]{2575B7} 0.73 & \cellcolor[HTML]{3383BE} 0.68 & \cellcolor[HTML]{BCD7EB} 0.28 & \cellcolor[HTML]{B1D2E7} 0.32 & \cellcolor[HTML]{3B8BC2} 0.65 \\
% sem\_0\_50\_100 & Worst & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{62A8D2} 0.52 & \cellcolor[HTML]{67ABD4} 0.51 & \cellcolor[HTML]{63A9D3} 0.52 & \cellcolor[HTML]{4292C6} 0.62 & \cellcolor[HTML]{3585BF} 0.67 & \cellcolor[HTML]{87BDDC} 0.43 & \cellcolor[HTML]{92C3DE} 0.40 & \cellcolor[HTML]{C7DBEF} 0.24 & \cellcolor[HTML]{C9DDF0} 0.23 & \cellcolor[HTML]{8FC1DD} 0.41 & \cellcolor[HTML]{549ECD} 0.57 & \cellcolor[HTML]{4A97C9} 0.60 & \cellcolor[HTML]{98C7DF} 0.39 & \cellcolor[HTML]{4C99CA} 0.59 & \cellcolor[HTML]{59A2CF} 0.55 & \cellcolor[HTML]{97C6DF} 0.39 & \cellcolor[HTML]{2A7AB9} 0.71 & \cellcolor[HTML]{A3CCE3} 0.36 & \cellcolor[HTML]{6AADD5} 0.50 & \cellcolor[HTML]{B1D2E7} 0.32 \\
% sem\_1\_20\_22 & Best & \cellcolor[HTML]{083978} 0.96 & \cellcolor[HTML]{08336F} 0.98 & \cellcolor[HTML]{083E80} 0.94 & \cellcolor[HTML]{083C7D} 0.95 & \cellcolor[HTML]{0E59A2} 0.84 & \cellcolor[HTML]{08509A} 0.88 & \cellcolor[HTML]{1765AB} 0.80 & \cellcolor[HTML]{1F6FB3} 0.75 & \cellcolor[HTML]{88BEDC} 0.43 & \cellcolor[HTML]{3383BE} 0.68 & \cellcolor[HTML]{519CCC} 0.58 & \cellcolor[HTML]{2070B4} 0.75 & \cellcolor[HTML]{08468C} 0.91 & \cellcolor[HTML]{9ECAE1} 0.37 & \cellcolor[HTML]{1765AB} 0.80 & \cellcolor[HTML]{98C7DF} 0.39 & \cellcolor[HTML]{135FA7} 0.82 & \cellcolor[HTML]{B6D4E9} 0.30 & \cellcolor[HTML]{7FB8DA} 0.45 & \cellcolor[HTML]{9DC9E0} 0.38 & \cellcolor[HTML]{3E8EC4} 0.64 \\
% sem\_1\_20\_22 & Worst & \cellcolor[HTML]{4E9ACA} 0.59 & \cellcolor[HTML]{3080BD} 0.69 & \cellcolor[HTML]{519CCC} 0.57 & \cellcolor[HTML]{4090C5} 0.63 & \cellcolor[HTML]{9AC7E0} 0.38 & \cellcolor[HTML]{519CCC} 0.58 & \cellcolor[HTML]{519CCC} 0.58 & \cellcolor[HTML]{6DAFD6} 0.49 & \cellcolor[HTML]{C0D8ED} 0.27 & \cellcolor[HTML]{C8DCEF} 0.24 & \cellcolor[HTML]{A3CCE3} 0.36 & \cellcolor[HTML]{4795C8} 0.61 & \cellcolor[HTML]{6BAED6} 0.50 & \cellcolor[HTML]{D6E5F4} 0.16 & \cellcolor[HTML]{92C3DE} 0.41 & \cellcolor[HTML]{A0CAE1} 0.37 & \cellcolor[HTML]{2B7BBA} 0.71 & \cellcolor[HTML]{9BC8E0} 0.38 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{3585BF} 0.67 & \cellcolor[HTML]{9BC8E0} 0.38 \\
% sem\_1\_50\_100 & Best & \cellcolor[HTML]{084991} 0.90 & \cellcolor[HTML]{084185} 0.93 & \cellcolor[HTML]{084083} 0.94 & \cellcolor[HTML]{084388} 0.93 & \cellcolor[HTML]{09539D} 0.87 & \cellcolor[HTML]{135FA7} 0.82 & \cellcolor[HTML]{084388} 0.92 & \cellcolor[HTML]{1967AD} 0.79 & \cellcolor[HTML]{2575B7} 0.73 & \cellcolor[HTML]{4C99CA} 0.59 & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{3D8DC3} 0.64 & \cellcolor[HTML]{08519C} 0.87 & \cellcolor[HTML]{1B6AAF} 0.77 & \cellcolor[HTML]{1562A9} 0.81 & \cellcolor[HTML]{7AB6D9} 0.46 & \cellcolor[HTML]{0D58A1} 0.85 & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{C4DAEE} 0.26 & \cellcolor[HTML]{D3E3F3} 0.18 & \cellcolor[HTML]{2F7FBC} 0.69 \\
% sem\_1\_50\_100 & Worst & \cellcolor[HTML]{87BDDC} 0.43 & \cellcolor[HTML]{ACD0E6} 0.33 & \cellcolor[HTML]{8BC0DD} 0.42 & \cellcolor[HTML]{69ACD5} 0.50 & \cellcolor[HTML]{92C3DE} 0.40 & \cellcolor[HTML]{83BBDB} 0.44 & \cellcolor[HTML]{A7CEE4} 0.34 & \cellcolor[HTML]{BAD6EA} 0.29 & \cellcolor[HTML]{A3CCE3} 0.36 & \cellcolor[HTML]{DAE8F5} 0.14 & \cellcolor[HTML]{B6D4E9} 0.30 & \cellcolor[HTML]{8DC0DD} 0.41 & \cellcolor[HTML]{88BEDC} 0.43 & \cellcolor[HTML]{D1E2F2} 0.19 & \cellcolor[HTML]{3585BF} 0.67 & \cellcolor[HTML]{61A7D2} 0.53 & \cellcolor[HTML]{549ECD} 0.57 & \cellcolor[HTML]{70B1D7} 0.49 & \cellcolor[HTML]{AFD1E6} 0.32 & \cellcolor[HTML]{9DC9E0} 0.38 & \cellcolor[HTML]{ABCFE5} 0.33 \\
% sem\_2\_100\_144 & Best & \cellcolor[HTML]{1C6BB0} 0.77 & \cellcolor[HTML]{1461A8} 0.81 & \cellcolor[HTML]{105CA4} 0.83 & \cellcolor[HTML]{0F5AA3} 0.84 & \cellcolor[HTML]{0E59A2} 0.84 & \cellcolor[HTML]{2878B8} 0.72 & \cellcolor[HTML]{1765AB} 0.79 & \cellcolor[HTML]{1F6FB3} 0.76 & \cellcolor[HTML]{559FCD} 0.57 & \cellcolor[HTML]{7FB8DA} 0.45 & \cellcolor[HTML]{5CA3D0} 0.55 & \cellcolor[HTML]{4795C8} 0.61 & \cellcolor[HTML]{3D8DC3} 0.64 & \cellcolor[HTML]{62A8D2} 0.53 & \cellcolor[HTML]{1E6EB2} 0.76 & \cellcolor[HTML]{8ABFDC} 0.42 & \cellcolor[HTML]{4191C5} 0.63 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{B5D3E9} 0.30 & \cellcolor[HTML]{7FB8DA} 0.45 & \cellcolor[HTML]{57A0CE} 0.56 \\
% sem\_2\_100\_144 & Worst & \cellcolor[HTML]{2E7EBC} 0.70 & \cellcolor[HTML]{2676B7} 0.73 & \cellcolor[HTML]{559FCD} 0.57 & \cellcolor[HTML]{3D8DC3} 0.64 & \cellcolor[HTML]{125EA6} 0.82 & \cellcolor[HTML]{3080BD} 0.69 & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{65AAD3} 0.52 & \cellcolor[HTML]{B4D3E8} 0.31 & \cellcolor[HTML]{AFD1E6} 0.32 & \cellcolor[HTML]{3787C0} 0.67 & \cellcolor[HTML]{77B4D8} 0.47 & \cellcolor[HTML]{6BAED6} 0.50 & \cellcolor[HTML]{A8CEE4} 0.34 & \cellcolor[HTML]{3C8CC3} 0.65 & \cellcolor[HTML]{83BBDB} 0.44 & \cellcolor[HTML]{4090C5} 0.63 & \cellcolor[HTML]{3181BD} 0.69 & \cellcolor[HTML]{90C2DE} 0.41 & \cellcolor[HTML]{3E8EC4} 0.64 & \cellcolor[HTML]{98C7DF} 0.39 \\
% sem\_2\_20\_19 & Best & \cellcolor[HTML]{083978} 0.96 & \cellcolor[HTML]{083471} 0.98 & \cellcolor[HTML]{084083} 0.93 & \cellcolor[HTML]{08458B} 0.92 & \cellcolor[HTML]{125EA6} 0.82 & \cellcolor[HTML]{1461A8} 0.81 & \cellcolor[HTML]{1E6DB2} 0.76 & \cellcolor[HTML]{08488F} 0.90 & \cellcolor[HTML]{8FC1DD} 0.41 & \cellcolor[HTML]{6FB0D6} 0.49 & \cellcolor[HTML]{4B98C9} 0.60 & \cellcolor[HTML]{1E6DB2} 0.76 & \cellcolor[HTML]{0A549E} 0.86 & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{2272B5} 0.74 & \cellcolor[HTML]{8DC0DD} 0.42 & \cellcolor[HTML]{105CA4} 0.83 & \cellcolor[HTML]{ADD0E6} 0.32 & \cellcolor[HTML]{A1CBE2} 0.36 & \cellcolor[HTML]{D7E6F4} 0.16 & \cellcolor[HTML]{A1CBE2} 0.36 \\
% sem\_2\_20\_19 & Worst & \cellcolor[HTML]{3989C1} 0.66 & \cellcolor[HTML]{2878B8} 0.72 & \cellcolor[HTML]{58A1CE} 0.56 & \cellcolor[HTML]{59A2CF} 0.55 & \cellcolor[HTML]{4A97C9} 0.60 & \cellcolor[HTML]{549ECD} 0.57 & \cellcolor[HTML]{2777B8} 0.72 & \cellcolor[HTML]{73B2D7} 0.48 & \cellcolor[HTML]{93C4DE} 0.40 & \cellcolor[HTML]{D6E5F4} 0.17 & \cellcolor[HTML]{C8DCEF} 0.24 & \cellcolor[HTML]{4795C8} 0.61 & \cellcolor[HTML]{61A7D2} 0.53 & \cellcolor[HTML]{C8DCEF} 0.23 & \cellcolor[HTML]{4795C8} 0.61 & \cellcolor[HTML]{6BAED6} 0.50 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{B1D2E7} 0.31 & \cellcolor[HTML]{A3CCE3} 0.36 & \cellcolor[HTML]{A1CBE2} 0.37 & \cellcolor[HTML]{B4D3E8} 0.31 \\
% sem\_2\_50\_100 & Best & \cellcolor[HTML]{0A549E} 0.86 & \cellcolor[HTML]{08509A} 0.88 & \cellcolor[HTML]{09539D} 0.87 & \cellcolor[HTML]{084C96} 0.89 & \cellcolor[HTML]{1765AB} 0.80 & \cellcolor[HTML]{0B559F} 0.86 & \cellcolor[HTML]{4694C7} 0.61 & \cellcolor[HTML]{1764AB} 0.80 & \cellcolor[HTML]{3383BE} 0.68 & \cellcolor[HTML]{4F9BCB} 0.59 & \cellcolor[HTML]{3E8EC4} 0.64 & \cellcolor[HTML]{1764AB} 0.80 & \cellcolor[HTML]{084B94} 0.89 & \cellcolor[HTML]{4090C5} 0.63 & \cellcolor[HTML]{0C56A0} 0.85 & \cellcolor[HTML]{92C3DE} 0.41 & \cellcolor[HTML]{08458B} 0.92 & \cellcolor[HTML]{3787C0} 0.67 & \cellcolor[HTML]{59A2CF} 0.55 & \cellcolor[HTML]{BBD6EB} 0.28 & \cellcolor[HTML]{2E7EBC} 0.70 \\
% sem\_2\_50\_100 & Worst & \cellcolor[HTML]{3989C1} 0.66 & \cellcolor[HTML]{3383BE} 0.68 & \cellcolor[HTML]{A7CEE4} 0.35 & \cellcolor[HTML]{6FB0D6} 0.49 & \cellcolor[HTML]{63A9D3} 0.52 & \cellcolor[HTML]{3484BF} 0.67 & \cellcolor[HTML]{3787C0} 0.67 & \cellcolor[HTML]{A8CEE4} 0.34 & \cellcolor[HTML]{B7D4EA} 0.29 & \cellcolor[HTML]{C6DBEF} 0.25 & \cellcolor[HTML]{9DC9E0} 0.38 & \cellcolor[HTML]{4090C5} 0.63 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{BBD6EB} 0.28 & \cellcolor[HTML]{4C99CA} 0.59 & \cellcolor[HTML]{77B4D8} 0.47 & \cellcolor[HTML]{7BB7D9} 0.46 & \cellcolor[HTML]{A7CEE4} 0.34 & \cellcolor[HTML]{3484BF} 0.67 & \cellcolor[HTML]{8ABFDC} 0.42 & \cellcolor[HTML]{93C4DE} 0.40 \\
% sem\_3\_100\_137 & Best & \cellcolor[HTML]{1D6CB1} 0.77 & \cellcolor[HTML]{0E59A2} 0.84 & \cellcolor[HTML]{09539D} 0.87 & \cellcolor[HTML]{084B94} 0.89 & \cellcolor[HTML]{0F5BA3} 0.83 & \cellcolor[HTML]{1F6FB3} 0.75 & \cellcolor[HTML]{1C6BB0} 0.77 & \cellcolor[HTML]{1967AD} 0.79 & \cellcolor[HTML]{80B9DA} 0.45 & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{1D6CB1} 0.77 & \cellcolor[HTML]{2E7EBC} 0.70 & \cellcolor[HTML]{2777B8} 0.72 & \cellcolor[HTML]{73B2D7} 0.48 & \cellcolor[HTML]{4B98C9} 0.60 & \cellcolor[HTML]{1663AA} 0.80 & \cellcolor[HTML]{C3D9EE} 0.26 & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{7FB8DA} 0.45 & \cellcolor[HTML]{3F8FC4} 0.63 \\
% sem\_3\_100\_137 & Worst & \cellcolor[HTML]{4A97C9} 0.60 & \cellcolor[HTML]{2575B7} 0.73 & \cellcolor[HTML]{77B4D8} 0.47 & \cellcolor[HTML]{4896C8} 0.60 & \cellcolor[HTML]{1461A8} 0.81 & \cellcolor[HTML]{2B7BBA} 0.71 & \cellcolor[HTML]{7FB8DA} 0.45 & \cellcolor[HTML]{B4D3E8} 0.31 & \cellcolor[HTML]{ACD0E6} 0.33 & \cellcolor[HTML]{BED7EC} 0.27 & \cellcolor[HTML]{4090C5} 0.63 & \cellcolor[HTML]{3C8CC3} 0.65 & \cellcolor[HTML]{6FB0D6} 0.49 & \cellcolor[HTML]{B1D2E7} 0.31 & \cellcolor[HTML]{3585BF} 0.67 & \cellcolor[HTML]{62A8D2} 0.53 & \cellcolor[HTML]{1663AA} 0.80 & \cellcolor[HTML]{83BBDB} 0.44 & \cellcolor[HTML]{59A2CF} 0.55 & \cellcolor[HTML]{69ACD5} 0.51 & \cellcolor[HTML]{C3D9EE} 0.26 \\
% sem\_5\_200\_194 & Best & \cellcolor[HTML]{083C7D} 0.95 & \cellcolor[HTML]{084489} 0.92 & \cellcolor[HTML]{08488F} 0.91 & \cellcolor[HTML]{09539D} 0.87 & \cellcolor[HTML]{2575B7} 0.73 & \cellcolor[HTML]{1C6BB0} 0.77 & \cellcolor[HTML]{2A7AB9} 0.71 & \cellcolor[HTML]{083C7D} 0.95 & \cellcolor[HTML]{62A8D2} 0.52 & \cellcolor[HTML]{58A1CE} 0.56 & \cellcolor[HTML]{A2CBE2} 0.36 & \cellcolor[HTML]{4B98C9} 0.60 & \cellcolor[HTML]{1967AD} 0.79 & \cellcolor[HTML]{2474B6} 0.74 & \cellcolor[HTML]{3181BD} 0.68 & \cellcolor[HTML]{9AC7E0} 0.38 & \cellcolor[HTML]{1E6EB2} 0.76 & \cellcolor[HTML]{1360A7} 0.82 & \cellcolor[HTML]{1A68AE} 0.78 & \cellcolor[HTML]{9BC8E0} 0.38 & \cellcolor[HTML]{67ABD4} 0.51 \\
% sem\_5\_200\_194 & Worst & \cellcolor[HTML]{539DCC} 0.57 & \cellcolor[HTML]{509BCB} 0.58 & \cellcolor[HTML]{70B1D7} 0.48 & \cellcolor[HTML]{58A1CE} 0.56 & \cellcolor[HTML]{4F9BCB} 0.58 & \cellcolor[HTML]{2E7EBC} 0.70 & \cellcolor[HTML]{6FB0D6} 0.49 & \cellcolor[HTML]{75B3D8} 0.47 & \cellcolor[HTML]{ABCFE5} 0.33 & \cellcolor[HTML]{C9DDF0} 0.23 & \cellcolor[HTML]{A7CEE4} 0.35 & \cellcolor[HTML]{4090C5} 0.63 & \cellcolor[HTML]{7FB8DA} 0.45 & \cellcolor[HTML]{B4D3E8} 0.31 & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{8ABFDC} 0.43 & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{08529C} 0.87 & \cellcolor[HTML]{08529C} 0.87 & \cellcolor[HTML]{3989C1} 0.66 & \cellcolor[HTML]{BBD6EB} 0.28 \\
% sem\_6\_200\_202 & Best & \cellcolor[HTML]{083A7A} 0.96 & \cellcolor[HTML]{084286} 0.93 & \cellcolor[HTML]{135FA7} 0.82 & \cellcolor[HTML]{0C56A0} 0.85 & \cellcolor[HTML]{1360A7} 0.81 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{61A7D2} 0.53 & \cellcolor[HTML]{1E6DB2} 0.77 & \cellcolor[HTML]{CCDFF1} 0.22 & \cellcolor[HTML]{61A7D2} 0.53 & \cellcolor[HTML]{6BAED6} 0.50 & \cellcolor[HTML]{1764AB} 0.80 & \cellcolor[HTML]{1B6AAF} 0.78 & \cellcolor[HTML]{8DC0DD} 0.42 & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{67ABD4} 0.51 & \cellcolor[HTML]{92C3DE} 0.40 & \cellcolor[HTML]{1E6EB2} 0.76 & \cellcolor[HTML]{D1E2F2} 0.19 & \cellcolor[HTML]{73B2D7} 0.48 & \cellcolor[HTML]{72B1D7} 0.48 \\
% sem\_6\_200\_202 & Worst & \cellcolor[HTML]{66AAD4} 0.51 & \cellcolor[HTML]{509BCB} 0.58 & \cellcolor[HTML]{57A0CE} 0.56 & \cellcolor[HTML]{3888C0} 0.66 & \cellcolor[HTML]{3181BD} 0.69 & \cellcolor[HTML]{2979B9} 0.71 & \cellcolor[HTML]{559FCD} 0.56 & \cellcolor[HTML]{1360A7} 0.81 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{B4D3E8} 0.31 & \cellcolor[HTML]{92C3DE} 0.41 & \cellcolor[HTML]{3282BE} 0.68 & \cellcolor[HTML]{65AAD3} 0.52 & \cellcolor[HTML]{87BDDC} 0.43 & \cellcolor[HTML]{2777B8} 0.73 & \cellcolor[HTML]{69ACD5} 0.51 & \cellcolor[HTML]{2E7EBC} 0.70 & \cellcolor[HTML]{08478E} 0.91 & \cellcolor[HTML]{A7CEE4} 0.35 & \cellcolor[HTML]{3E8EC4} 0.64 & \cellcolor[HTML]{BFD8EC} 0.27 \\
% sem\_9\_100\_131 & Best & \cellcolor[HTML]{0F5BA3} 0.83 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{084C96} 0.89 & \cellcolor[HTML]{084B94} 0.89 & \cellcolor[HTML]{4191C5} 0.63 & \cellcolor[HTML]{4C99CA} 0.59 & \cellcolor[HTML]{135FA7} 0.82 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{66AAD4} 0.51 & \cellcolor[HTML]{519CCC} 0.58 & \cellcolor[HTML]{9BC8E0} 0.38 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{2575B7} 0.73 & \cellcolor[HTML]{2070B4} 0.75 & \cellcolor[HTML]{3383BE} 0.68 & \cellcolor[HTML]{9DC9E0} 0.38 & \cellcolor[HTML]{2B7BBA} 0.71 & \cellcolor[HTML]{3383BE} 0.68 & \cellcolor[HTML]{92C3DE} 0.40 & \cellcolor[HTML]{B6D4E9} 0.30 & \cellcolor[HTML]{519CCC} 0.58 \\
% sem\_9\_100\_131 & Worst & \cellcolor[HTML]{2F7FBC} 0.69 & \cellcolor[HTML]{58A1CE} 0.56 & \cellcolor[HTML]{90C2DE} 0.41 & \cellcolor[HTML]{6BAED6} 0.50 & \cellcolor[HTML]{084C96} 0.89 & \cellcolor[HTML]{1E6EB2} 0.76 & \cellcolor[HTML]{2373B6} 0.74 & \cellcolor[HTML]{A6CDE3} 0.35 & \cellcolor[HTML]{B2D2E8} 0.31 & \cellcolor[HTML]{AFD1E6} 0.32 & \cellcolor[HTML]{4A97C9} 0.60 & \cellcolor[HTML]{4B98C9} 0.59 & \cellcolor[HTML]{6DAFD6} 0.49 & \cellcolor[HTML]{D1E2F2} 0.19 & \cellcolor[HTML]{3282BE} 0.68 & \cellcolor[HTML]{A7CEE4} 0.35 & \cellcolor[HTML]{3C8CC3} 0.65 & \cellcolor[HTML]{3787C0} 0.67 & \cellcolor[HTML]{7AB6D9} 0.46 & \cellcolor[HTML]{BCD7EB} 0.28 & \cellcolor[HTML]{B2D2E8} 0.31 \\
% sem\_9\_200\_150 & Best & \cellcolor[HTML]{084083} 0.94 & \cellcolor[HTML]{084286} 0.93 & \cellcolor[HTML]{125EA6} 0.82 & \cellcolor[HTML]{0F5BA3} 0.83 & \cellcolor[HTML]{1461A8} 0.81 & \cellcolor[HTML]{1461A8} 0.81 & \cellcolor[HTML]{084E97} 0.89 & \cellcolor[HTML]{08458B} 0.91 & \cellcolor[HTML]{A5CDE3} 0.35 & \cellcolor[HTML]{63A9D3} 0.52 & \cellcolor[HTML]{A8CEE4} 0.34 & \cellcolor[HTML]{2676B7} 0.73 & \cellcolor[HTML]{1967AD} 0.79 & \cellcolor[HTML]{1C6BB0} 0.77 & \cellcolor[HTML]{2676B7} 0.73 & \cellcolor[HTML]{9ECAE1} 0.37 & \cellcolor[HTML]{08478E} 0.91 & \cellcolor[HTML]{D2E3F3} 0.18 & \cellcolor[HTML]{BFD8EC} 0.27 & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{509BCB} 0.58 \\
% sem\_9\_200\_150 & Worst & \cellcolor[HTML]{A3CCE3} 0.36 & \cellcolor[HTML]{61A7D2} 0.53 & \cellcolor[HTML]{6DAFD6} 0.50 & \cellcolor[HTML]{4090C5} 0.63 & \cellcolor[HTML]{66AAD4} 0.52 & \cellcolor[HTML]{2A7AB9} 0.71 & \cellcolor[HTML]{C8DCEF} 0.24 & \cellcolor[HTML]{C5DAEE} 0.25 & \cellcolor[HTML]{2C7CBB} 0.71 & \cellcolor[HTML]{D1E2F2} 0.19 & \cellcolor[HTML]{8FC1DD} 0.41 & \cellcolor[HTML]{4A97C9} 0.60 & \cellcolor[HTML]{88BEDC} 0.43 & \cellcolor[HTML]{CEE0F1} 0.20 & \cellcolor[HTML]{3989C1} 0.66 & \cellcolor[HTML]{9BC8E0} 0.38 & \cellcolor[HTML]{A7CEE4} 0.35 & \cellcolor[HTML]{AACFE5} 0.34 & \cellcolor[HTML]{509BCB} 0.58 & \cellcolor[HTML]{08529C} 0.87 & \cellcolor[HTML]{CCDFF1} 0.22 \\
% tree\_100\_2 & Best & \cellcolor[HTML]{2979B9} 0.72 & \cellcolor[HTML]{2D7DBB} 0.70 & \cellcolor[HTML]{2171B5} 0.75 & \cellcolor[HTML]{1A68AE} 0.78 & \cellcolor[HTML]{1765AB} 0.79 & \cellcolor[HTML]{1C6BB0} 0.77 & \cellcolor[HTML]{084388} 0.93 & \cellcolor[HTML]{084388} 0.92 & \cellcolor[HTML]{D1E2F2} 0.19 & \cellcolor[HTML]{5AA3CF} 0.55 & \cellcolor[HTML]{87BDDC} 0.43 & \cellcolor[HTML]{2A7AB9} 0.71 & \cellcolor[HTML]{1967AD} 0.79 & \cellcolor[HTML]{1D6CB1} 0.77 & \cellcolor[HTML]{8BC0DD} 0.42 & \cellcolor[HTML]{7BB7D9} 0.46 & \cellcolor[HTML]{83BBDB} 0.44 & \cellcolor[HTML]{1967AD} 0.79 & \cellcolor[HTML]{97C6DF} 0.39 & \cellcolor[HTML]{ADD0E6} 0.33 & \cellcolor[HTML]{5EA5D1} 0.54 \\
% tree\_100\_2 & Worst & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{77B4D8} 0.47 & \cellcolor[HTML]{A5CDE3} 0.35 & \cellcolor[HTML]{73B2D7} 0.48 & \cellcolor[HTML]{83BBDB} 0.44 & \cellcolor[HTML]{72B1D7} 0.48 & \cellcolor[HTML]{A6CDE3} 0.35 & \cellcolor[HTML]{D6E5F4} 0.17 & \cellcolor[HTML]{C9DDF0} 0.23 & \cellcolor[HTML]{B0D1E7} 0.32 & \cellcolor[HTML]{4292C6} 0.62 & \cellcolor[HTML]{1764AB} 0.80 & \cellcolor[HTML]{559FCD} 0.56 & \cellcolor[HTML]{BCD7EB} 0.28 & \cellcolor[HTML]{115DA5} 0.83 & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{08458B} 0.91 & \cellcolor[HTML]{1B6AAF} 0.78 & \cellcolor[HTML]{3484BF} 0.67 & \cellcolor[HTML]{85BCDB} 0.44 & \cellcolor[HTML]{BFD8EC} 0.27 \\
% tree\_200\_2 & Best & \cellcolor[HTML]{0F5BA3} 0.83 & \cellcolor[HTML]{1E6DB2} 0.76 & \cellcolor[HTML]{0F5AA3} 0.84 & \cellcolor[HTML]{1764AB} 0.80 & \cellcolor[HTML]{1562A9} 0.81 & \cellcolor[HTML]{2C7CBB} 0.70 & \cellcolor[HTML]{08509A} 0.88 & \cellcolor[HTML]{084991} 0.90 & \cellcolor[HTML]{C4DAEE} 0.26 & \cellcolor[HTML]{61A7D2} 0.53 & \cellcolor[HTML]{73B2D7} 0.48 & \cellcolor[HTML]{3F8FC4} 0.63 & \cellcolor[HTML]{2373B6} 0.74 & \cellcolor[HTML]{2979B9} 0.72 & \cellcolor[HTML]{6FB0D6} 0.49 & \cellcolor[HTML]{AFD1E6} 0.32 & \cellcolor[HTML]{93C4DE} 0.40 & \cellcolor[HTML]{ABCFE5} 0.33 & \cellcolor[HTML]{70B1D7} 0.49 & \cellcolor[HTML]{CBDEF0} 0.23 & \cellcolor[HTML]{2878B8} 0.72 \\
% tree\_200\_2 & Worst & \cellcolor[HTML]{3484BF} 0.67 & \cellcolor[HTML]{3F8FC4} 0.64 & \cellcolor[HTML]{73B2D7} 0.48 & \cellcolor[HTML]{60A6D1} 0.53 & \cellcolor[HTML]{58A1CE} 0.56 & \cellcolor[HTML]{60A6D1} 0.53 & \cellcolor[HTML]{93C4DE} 0.40 & \cellcolor[HTML]{C3D9EE} 0.26 & \cellcolor[HTML]{C0D8ED} 0.27 & \cellcolor[HTML]{8FC1DD} 0.41 & \cellcolor[HTML]{4694C7} 0.61 & \cellcolor[HTML]{4393C6} 0.62 & \cellcolor[HTML]{3F8FC4} 0.63 & \cellcolor[HTML]{CBDEF0} 0.22 & \cellcolor[HTML]{2B7BBA} 0.71 & \cellcolor[HTML]{B0D1E7} 0.32 & \cellcolor[HTML]{2474B6} 0.73 & \cellcolor[HTML]{A5CDE3} 0.35 & \cellcolor[HTML]{3A8AC1} 0.65 & \cellcolor[HTML]{C3D9EE} 0.26 & \cellcolor[HTML]{ACD0E6} 0.33 \\
% tree\_20\_0 & Best & \cellcolor[HTML]{08316C} 0.99 & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{08306B} 1.00 & \cellcolor[HTML]{084388} 0.92 & \cellcolor[HTML]{F7FBFF} 0.00 & \cellcolor[HTML]{8BC0DD} 0.42 & \cellcolor[HTML]{92C3DE} 0.41 & \cellcolor[HTML]{3F8FC4} 0.63 & \cellcolor[HTML]{135FA7} 0.82 & \cellcolor[HTML]{3B8BC2} 0.65 & \cellcolor[HTML]{1562A9} 0.81 & \cellcolor[HTML]{ABCFE5} 0.33 & \cellcolor[HTML]{115DA5} 0.83 & \cellcolor[HTML]{C7DBEF} 0.24 & \cellcolor[HTML]{C3D9EE} 0.26 & \cellcolor[HTML]{A5CDE3} 0.35 & \cellcolor[HTML]{2D7DBB} 0.70 \\
% tree\_20\_0 & Worst & \cellcolor[HTML]{D7E6F4} 0.16 & \cellcolor[HTML]{8DC0DD} 0.41 & \cellcolor[HTML]{9AC7E0} 0.39 & \cellcolor[HTML]{2777B8} 0.73 & \cellcolor[HTML]{ACD0E6} 0.33 & \cellcolor[HTML]{6BAED6} 0.50 & \cellcolor[HTML]{95C5DF} 0.40 & \cellcolor[HTML]{C4DAEE} 0.26 & \cellcolor[HTML]{559FCD} 0.57 & \cellcolor[HTML]{DBE9F6} 0.14 & \cellcolor[HTML]{4090C5} 0.63 & \cellcolor[HTML]{2777B8} 0.73 & \cellcolor[HTML]{7AB6D9} 0.46 & \cellcolor[HTML]{D7E6F4} 0.16 & \cellcolor[HTML]{78B5D8} 0.47 & \cellcolor[HTML]{A5CDE3} 0.35 & \cellcolor[HTML]{AACFE5} 0.34 & \cellcolor[HTML]{8DC0DD} 0.41 & \cellcolor[HTML]{3B8BC2} 0.65 & \cellcolor[HTML]{C8DCEF} 0.24 & \cellcolor[HTML]{DDEAF6} 0.13 \\
% tree\_50\_2 & Best & \cellcolor[HTML]{08509A} 0.88 & \cellcolor[HTML]{083B7B} 0.95 & \cellcolor[HTML]{09539D} 0.86 & \cellcolor[HTML]{08509A} 0.88 & \cellcolor[HTML]{135FA7} 0.82 & \cellcolor[HTML]{1A68AE} 0.78 & \cellcolor[HTML]{084185} 0.93 & \cellcolor[HTML]{084991} 0.90 & \cellcolor[HTML]{6FB0D6} 0.49 & \cellcolor[HTML]{83BBDB} 0.44 & \cellcolor[HTML]{92C3DE} 0.41 & \cellcolor[HTML]{3F8FC4} 0.63 & \cellcolor[HTML]{3484BF} 0.67 & \cellcolor[HTML]{4292C6} 0.62 & \cellcolor[HTML]{2878B8} 0.72 & \cellcolor[HTML]{A8CEE4} 0.34 & \cellcolor[HTML]{2272B5} 0.74 & \cellcolor[HTML]{75B3D8} 0.48 & \cellcolor[HTML]{80B9DA} 0.45 & \cellcolor[HTML]{BCD7EB} 0.28 & \cellcolor[HTML]{4B98C9} 0.60 \\
% tree\_50\_2 & Worst & \cellcolor[HTML]{67ABD4} 0.51 & \cellcolor[HTML]{2777B8} 0.73 & \cellcolor[HTML]{9AC7E0} 0.39 & \cellcolor[HTML]{5AA3CF} 0.55 & \cellcolor[HTML]{AACFE5} 0.34 & \cellcolor[HTML]{97C6DF} 0.39 & \cellcolor[HTML]{B5D3E9} 0.30 & \cellcolor[HTML]{E5EFF9} 0.09 & \cellcolor[HTML]{519CCC} 0.57 & \cellcolor[HTML]{B7D4EA} 0.30 & \cellcolor[HTML]{4E9ACA} 0.59 & \cellcolor[HTML]{559FCD} 0.56 & \cellcolor[HTML]{72B1D7} 0.48 & \cellcolor[HTML]{E1EDF8} 0.11 & \cellcolor[HTML]{1B6AAF} 0.77 & \cellcolor[HTML]{ACD0E6} 0.33 & \cellcolor[HTML]{084E97} 0.88 & \cellcolor[HTML]{73B2D7} 0.48 & \cellcolor[HTML]{125EA6} 0.82 & \cellcolor[HTML]{7DB8D9} 0.46 & \cellcolor[HTML]{D4E4F3} 0.18 \\
% \bottomrule
% \end{tabular}
% \end{tiny}
% \label{tab:my_label}
% \end{table}
